Online Min-Max Paging

Motivated by fairness requirements in communication networks, we introduce a natural variant of the online paging problem, called \textit{min-max} paging, where the objective is to minimize the maximum number of faults on any page. While the classical paging problem, whose objective is to minimize the total number of faults, admits $k$-competitive deterministic and $O(\log k)$-competitive randomized algorithms, we show that min-max paging does not admit a $c(k)$-competitive algorithm for any function $c$. Specifically, we prove that the randomized competitive ratio of min-max paging is $\Omega(\log(n))$ and its deterministic competitive ratio is $\Omega(k\log(n)/\log(k))$, where $n$ is the total number of pages ever requested. We design a fractional algorithm for paging with a more general objective -- minimize the value of an $n$-variate differentiable convex function applied to the vector of the number of faults on each page. This gives an $O(\log(n)\log(k))$-competitive fractional algorithm for min-max paging. We show how to round such a fractional algorithm with at most a $k$ factor loss in the competitive ratio, resulting in a deterministic $O(k\log(n)\log(k))$-competitive algorithm for min-max paging. This matches our lower bound modulo a $\mathrm{poly}(\log(k))$ factor. We also give a randomized rounding algorithm that results in a $O(\log^2 n \log k)$-competitive algorithm.

==> MinMax (Fair) Paging/abstract.tex <==
Motivated by fairness requirements in communication networks, 
we introduce a natural variant of the online paging problem, called \textit{min-max} paging, where the objective is to minimize the maximum number of faults on any page. While the classical paging problem, whose objective is to minimize the total number of faults, admits $k$-competitive deterministic and $O(\log k)$-competitive randomized algorithms, we show that min-max paging does not admit a $c(k)$-competitive algorithm for any function $c$. Specifically, we prove that the randomized competitive ratio of min-max paging is $\Omega(\log(n))$ and its deterministic competitive ratio is $\Omega(k\log(n)/\log(k))$, where $n$ is the total number of pages ever requested.

We design a fractional algorithm for paging with a more general objective -- minimize the value of an $n$-variate differentiable convex function applied to the vector of the number of faults on each page. This gives an $O(\log(n)\log(k))$-competitive fractional algorithm for min-max paging. We show how to round such a fractional algorithm with at most a $k$ factor loss in the competitive ratio, resulting in a deterministic $O(k\log(n)\log(k))$-competitive algorithm for min-max paging. This matches our lower bound modulo a $\poly(\log(k))$ factor.
We also give a randomized rounding algorithm that results in a $O(\log^2 n \log k)$-competitive algorithm.


==> MinMax (Fair) Paging/app_detlb.tex <==
\input{detlb.tex}



%In this section, we will show that any deterministic algorithm for min-max paging is $\Omega(\frac{k}{\log k} \log n)$ competitive. This result separates min-max paging from classical paging and its variants, which are generally $\Theta(k)$ competitive.
% We begin by showing a lower bound of $\frac{k}{2}$, which we then strengthen
% to the stated bound.

For any paging algorithm ALG and any request sequence $\sigma$, we define $\cost(\ALG, \sigma, p, t)$ to be the the number of page faults incurred on page $p$ after processing the first $t$ requests of $\sigma$. Furthermore, we define \[\cost(\ALG, \sigma) = \max_{p \in P} \cost(\ALG, \sigma, p, T),\] to be the overall cost incurred by ALG while processing request sequence $\sigma$.

The optimal offline algorithm OPT for min-max paging is not known to us, so we use Algorithm~\ref{greedylfd} (GreedyLFD) to obtain an upper bound on the cost of OPT. Intuitively, this algorithm avoids increasing its maximum cost for as long as possible by greedily keeping the most expensive pages in its cache. As GreedyLFD is an offline algorithm, it has access to the complete request sequence $\sigma$ and can always eject the page that is \emph{furthest in the future}. That is, in round $t$, it ejects the page $p \in C$ whose next occurrence comes last in the remainder of $\sigma$ after $t$. If a page does not occur in the remainder of $\sigma$, it is treated as being infinitely far in the future, and the algorithm will always prefer to eject this page over one that will still occur in $\sigma$.

\begin{algorithm}
  \caption{The offline algorithm GreedyLFD}\label{greedylfd}
  \begin{algorithmic}[1]
    \Procedure{GreedyLFD}{$\sigma$} \State $C \gets \emptyset$
    \Comment{Initialize the cache.}  \State $t \gets 1$ \For{$p \in P$} \State
    $c_p \gets 0$ \Comment{Counter variables for the number of faults on page
      $p$. At any point in time $c_p = cost(GreedyLFD, \sigma, p, t)$.}  \EndFor
    \While{$t < T$} \If{the $t$th element, say $p_t$, of $\sigma$ is not in $C$}
    \State $c_p \gets c_p + 1$ \If{$|C| < k$} \State $C \gets C \cup \{p\}$
    \Else \State $S \gets \{q \in C \mid c_q < \max_r c_r \}$ \Comment{Obtain
      the set of pages whose cost is less than the current maximum.}

    \If{$S = \emptyset$} \Comment{This happens if all pages in $C$ are of the
      same cost.}  \State $S \gets C$ \EndIf

    \State Evict $q \in S$ which next occurs farthest in the future.  \EndIf
    \EndIf \State $t \gets t+1$ \EndWhile \EndProcedure
  \end{algorithmic}
\end{algorithm}

\begin{lemma}\label{lfdlb}
  Let $\sigma$ be a request sequence for min-max paging using $k+1$ unique  pages. Then
  \[
    \cost(GreedyLFD, \sigma) \le \frac{2 (\len(\sigma) - 2k - 1)}{2k + k
      (k+1)}+2.
  \]
\end{lemma}
\begin{proof}
  We fix $\sigma$ to be an arbitrary request sequence of length $T$ using pages from the set $P = \{p_1, p_2, \dots, p_{k+1}\}$. Let
  \[
  t_i = \min \left\{t \in [T] \mid \max_{p \in P} \cost(GreedyLFD, \sigma, p,t) \ge i \right\}
  \]
  be the first time GreedyLFD faults on a page for the $i$th time. We note that at time $t_i$, there is only one page of cost $i$.

  Furthermore, we note that $t_1 = 1$, as the algorithm starts with an empty cache and $t_2 \ge 2k+1$, as the algorithm will fault on the first $k+1$ distinct pages it encounters, and it will then eject the page of cost $1$ which occurs farthest in the future. As there are $k$ pages in its cache, at least one page will not occur in the next $k-1$ time steps, so the shortest sequence that can cause GreedyLFD to fault two times on a single page is of length $2k+1$.

  We now show $t_{i+1} \ge t_i + k + \frac{k(k+1)}{2}$ for all $i \ge 2$. Let us fix $i \geq 2$ and assume we are currently at time $t_{i}$. This means that there exists some page $p \in P$ for which $\cost(GreedyLFD, \sigma, p, t_i) = i$ and it is the only page of cost $i$. In order to make room for $p$, GreedyLFD will evict a page of cost at most $i-1$ from its cache. As there are $k$ such pages in the cache at time $t_i$, at least one of them will not occur for the next $k-1$ requests. As there are only $k+1$ pages in total, this means that the next page fault occurs at time $t_i + k$ or later.

  In general, when the $j$th page of cost $i$ is added to GreedyLFD's cache at time $t_{i,j}$, there are $k-j+1$ pages of cost at most $i-1$ in its cache, and so the next page fault will not occur until time $t_{i,j} + k - j +1$, which gives a lower bound on $t_{i,j+1}$. Note that $t_{i,1} = t_i$

  As GreedyLFD's cost can only increase to $i+1$ once it evicts a page of cost $i$, we find that $t_{i+1}$ must occur after $k$ pages of cost $i$ have been added to its cache. GreedyLFD can choose which of the $k$ pages of cost $i$ to evict, so we find $t_{i+1} \ge t_{i,k} + k$. This yields
  \[
    t_{i+1} \ge t_{i,k} + k \ge t_{i,k-1} + k + 1 \ge t_{i,k-2} + k + 1 + 2 \ge
    \dots \ge t_{i} + k + \sum_{i=1}^k i.
  \]

  By expanding the recurrence for $i \ge 2$, we find that
  \[
  _i \ge (i-2) \left(k + \frac{k(k+1)}{2}\right) + 2k + 1.
  \]

  Using this expression, we derive an upper bound on $\cost(GreedyLFD, \sigma)$, by finding the minimum $i$ for which $\len(\sigma) \le t_i$. From our expression we find that $t_i \ge \len(\sigma)$ if $i \ge \frac{2(T - 2k - 1)}{2k + k(k+1)} + 2$, and so
  \[
    \cost(GreedyLFD, \sigma) \le \frac{2(\len(\sigma)-2k-1)}{2k + k(k+1)}+2.
  \]
\end{proof}

%\sag{Max, is this necessary?  Can we not directly state $\log n$ LB?} \mx{Yes, we need to show k-competitiveness as we use it as an ingredient in the $k \log n$ lower bound.}
\begin{lemma}
  Any deterministic algorithm ALG for min-max paging with cache size $k$ is at least $\frac{k}{2}$-competitive.
\end{lemma}
\begin{proof}
  Let $n = k+1$, that is $P = \{p_1, p_2, \dots, p_{k+1}\}$. We initialize ALG and GreedyLFD with empty caches. Once ALG's cache is full, at any time step $t$, there is always one page that is not present in the cache. The adversary's strategy is always to request this page. We call this the \emph{cruel} strategy. Since ALG is deterministic, the adversary always knows which page ALG will evict from its cache if a page fault occurs, so such a sequence must always exist.

  \begin{algorithm}
    \caption{An algorithm to generate an adversarial sequence for ALG of length
      $T \ge k+1$, on which ALG faults $T$ times.}\label{cruel}
    \begin{algorithmic}[1]
      \State \Output pages $p_1, p_2, \dots, p_{k+1}$ \State $i \gets k+1$
      \While{$i < T$} \State $p \gets $ the page $p_i$ which is currently not in
      the cache of ALG; \State \Output $p$ \State $i \gets i+1$ \EndWhile
    \end{algorithmic}
  \end{algorithm}

  Let $\sigma$ be a sequence of length $T$ generated by the cruel strategy of Algorithm~\ref{cruel}.  We note that $\sigma$ causes a page fault at every step, so the total number of page faults incurred by ALG will be $T$. By a simple averaging argument, there must be at least one page that has incurred $\frac{T}{k+1}$ page faults and so $\frac{T}{k+1} \le cost(ALG, \sigma)$. On the other hand, by Lemma \ref{lfdlb}, GreedyLFD will incur a cost of at most $\frac{2(T-2k-1)}{2k+k(k+1)}+2$ while processing $\sigma$. This immediately yields
  \begin{equation*}
    \cost(\OPT, \sigma) \le \cost(GreedyLFD, \sigma) \le \frac{2(T-2k-2)}{2k + k(k+1)} + 2 \le \frac{2T}{k(k+1)} + 2\le \frac{2}{k} \cost(ALG, \sigma) + 2,
  \end{equation*}
  and so the competitive ratio is $\frac{cost(ALG, \sigma)}{\cost(OPT, \sigma)} \ge \frac{k}{2}$, since the constant vanishes as the cost grows large.
\end{proof}

Finally, we strengthen the lower bound to $\Omega(\frac{k}{\log k} \log n)$, introducing a dependence on the number of pages. We do this using the strategy presented in Algorithm~\ref{detlbnew}.

\begin{algorithm}
  \caption{An adversarial strategy for min-max paging}\label{detlbnew}
  \begin{algorithmic}[1]
    \State Let $L_m=\{p^m_0,\ldots,p^m_{n-1}\}$ be a set of $n=(k+1)^m$ pages.
    \For{$\ell$ $=$ $m$ to $1$} \State $L_{\ell-1}\gets\emptyset$.  \For{$i$ $=$
      $0$ to $(k+1)^{\ell-1}-1$} \State Use the cruel strategy of Algorithm
    \ref{cruel} on the set of $k+1$ pages
    $\{p^\ell_{(k+1)i}, p^\ell_{(k+1)i+1}, \dots, p^\ell_{(k+1)i+k} \}$ until one
    page, say $p'$, has incurred $N$ page faults since the start of this loop.
    \State $p^{\ell-1}_i$ $\gets$ $p'$ \State
    $L_{\ell-1} \gets L_{\ell-1} \cup \{ p^{\ell-1}_i \}$ \EndFor \EndFor
  \end{algorithmic}
\end{algorithm}

Intuitively, our strategy consists of splitting the $n = (k+1)^m$ pages into $(k+1)^{m-1}$ disjoint sets of $k+1$ variables. We then present the algorithm ALG with a cruel sequence for each set until one of the pages reaches cost $N$. We repeat this process layer by layer until we obtain one final page. ALG will have faulted $mN$ times on this page, while OPT will have faulted no more than roughly $\frac{N}{k} + m$ times on any page.

\detlb*
% \begin{theorem}
%   Any deterministic algorithm ALG for min-max paging with cache size $k$ is at least $\frac{k-1}{2} \log_{k+1} n$-competitive.
% \end{theorem}
\begin{proof}
  We use the strategy defined in Algorithm \ref{detlbnew} to generate our request sequence. We observe that at the beginning of iteration $\ell$ of the outer for-loop in Algorithm \ref{detlbnew}, ALG will have faulted $(m-\ell)N$ times on each page in $\{p^{\ell}_0, \dots, p^{\ell}_{(k+1)^{\ell}-1}\}$, because we only add a page to the next level once it has incurred $N$ faults during the current level. Hence, once ALG has processed the complete sequence provided by Algorithm \ref{detlbnew}, it has cost $mN$, witnessed by page $p_0^0$.

  On the other hand, while processing the $i$th set of variables in the inner loop, the optimal offline algorithm OPT will keep page $p'$ in its cache. When $p'$ is requested for the first time in this iteration of the loop, OPT will fault once on $p'$. Afterward, $p'$ will remain in the cache of OPT until the current iteration of the inner loop finishes, incurring no more cost.

  This shows that OPT will have cost $m - \ell$ for each page $p_0^\ell, \dots, p_{(k+1)^{\ell}- 1}^\ell$ at the beginning of the $\ell$th iteration of the outer loop.

  During an iteration of the inner loop, we use the remaining $k-1$ slots in OPT's cache, which are not occupied by $p'$, to process the remaining $k$ pages in each iteration. As the cruel sequence causes ALG to fault on every request and we end it as soon as one page has faulted $N$ times, each of the remaining pages may be requested $N-1$ times. It follows that the sub-sequence $\sigma'$ of the cruel sequence, defined on the remaining $k$ pages, is of length at most $k(N-1)$. By Lemma \ref{lfdlb}, we get $\cost(\OPT, \sigma') \le \frac{2(k(N-1) - 2(k-1) - 1)}{2(k-1) + (k-1)k}+2 \le \frac{2(N-1)}{k-1} + 2$.

  Thus we find that for any page $p$, the total cost consists of the level it is raised to plus the cost incurred while processing $\sigma'$ on its last level and thus $\cost(OPT, \sigma, p, T) \le m + \frac{2(N-1)}{k-1}+2$ and so
  \[
    \frac{\cost(ALG, \rho)}{\cost(OPT,\rho)} \ge \frac{mN}{m + 2 +
      \frac{2(N-1)}{k-1}} = \frac{(k-1)mN}{(k-1)(m+2) + 2(N-1)}.
  \]
  As $N$ grows large, the right hand side will converge to $\frac{(k-1)m}{2} = \frac{k-1}{2} \log_{k+1} n$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/app_lb.tex <==
\section{Further Details for Lower Bounds}
\label{app:lb}
This section shows the complete details for the deterministic lower bound for min-max paging. We begin with a proof of the lower bound for $k=2$, which neatly highlights the core construction lying at the heart of the lower bound.

\input{app_detlb.tex}

%\input{app_randlb.tex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/app_proofs.tex <==
\section{Deferred Proofs}

This section contains some deferred proofs from the paper.

\fenchelmonotone*
\begin{proof}
Indeed, let $c \in \R_{+}^T$, then 
\[
f^*(y) = \sup_{w \in \R_{+}^T} \langle y, w \rangle - f(w) \le \sup_{w
\in \R_{+}^T} \langle y, w \rangle + \langle c, w \rangle - f(w) = f^*(y +
c),
\]
as $\langle c, w\rangle$ is always non-negative.
\end{proof}

\weakduality*
\begin{proof} 
Let $b = \begin{bmatrix} B(1)-k \\ \vdots \\ B(T) - k \end{bmatrix}$. As $x$ is feasible, it must satisfy $A x \ge b$, which gives $b - Ax \le \zeros$, and similarly from $x \le \ones$, we get $x - \ones \le \zeros$. As all entries are negative, taking the inner product of these vectors with the non-negative vectors $y$ and $z$, respectively, will yield a negative number. Hence, we get the first inequality in the following chain of inequalities:
\begin{align*}
  f(x) &\ge f(x) + y^\top ((|B(t)|-k) \ones - Ax) + z^\top (x -\ones) \\
       &= \sum_{t = 1}^{T} (|B(t)|-k)y_t - \sum_{p=1}^{n} \sum_{j=1}^{r(p,T)} z_{p,j} - (y^\top Ax -z^\top x - f(x))\\
       &= \sum_{t=1}^{T} (|B(t)|-k)y_t -  \sum_{p=1}^{n} \sum_{j=1}^{r(p,T)} z_{p,j} -(\langle A^\top y - z, x\rangle - f(x))\\
       &\ge \sum_{t=1}^{T} (|B(t)|-k)y_t -  \sum_{p=1}^{n} \sum_{j=1}^{r(p,T)} z_{p,j} - \sup_{w \in \R_+^T} (\langle A^\top y - z, w\rangle -f(w))\\
       &= \sum_{t=1}^{T} (|B(t)|-k)y_t -  \sum_{p=1}^{n} \sum_{j=1}^{r(p,T)} z_{p,j} - f^*(A^\top y -z).\\
\end{align*}
All equalities are obtained via simple rearranging of terms, and the final inequality is due to the definition of the supremum.
\end{proof}

\xlowerbound*
\begin{proof}
First, observe that $x_{p,j}$ starts increasing at time $\tau(t(p,j))$, the time at which we finish processing the $j$'th request to $p$. $x_{p,j}$ keeps increasing until one of the two events happens: $x_{p,j}$ reaches $1$, or we get the next request to $p$, after which it remains constant till the end. Let $\tau^{\text{end}}$ denote the time at which either of these events happens.

For $\tau\in[\tau(t(p,j)),\tau^{\text{end}})$, we have
\[\frac{dx_{p,j}(\tau)}{d\tau}=s_{p,j}(\tau)\cdot\left(x_{p,j}(\tau)+\frac{1}{k}\right)\geq s_{p,j}'\cdot\left(x_{p,j}(\tau)+\frac{1}{k}\right)\text{,}\]
and therefore,
\[\frac{1}{s_{p,j}'}\frac{d}{d\tau}\ln\left(x_{p,j}(\tau)+\frac{1}{k}\right)=\frac{1}{s_{p,j}'\cdot(x_{p,j}(\tau)+1/k)}\cdot\frac{dx_{p,j}(\tau)}{d\tau}\geq1\text{.}\]
Integrating over the interval $[\tau(t(p,j)),\tau^{\text{end}})$, we get,
\begin{equation}\label{eqn_x}
\frac{1}{s_{p,j}'}\ln\left(\frac{\bar{x}_{p,j}+1/k}{1/k}\right)\geq\tau^{\text{end}}-\tau(t(p,j))\text{.}
\end{equation}

Next, observe that the variable $y_t$ starts increasing from $0$ at the uniform rate $r$ at time $\tau(t-1)$ and stops increasing at time $\tau(t)$. Thus, $\bar{y}_t=r\cdot(\tau(t)-\tau(t-1))$. Summing over all $t$ from $t(p,j)+1$ to $t(p,j+1)-1$, we get,
\begin{equation}\label{eqn_y}
\frac{1}{r}\cdot\left(\sum_{t=t(p,j)+1}^{t(p,j+1)-1}\bar{y}_t\right)=\tau(t(p,j+1)-1)-\tau(t(p,j))\text{.}
\end{equation}

Finally, consider the variable $z_{p,j}$. If $x_{p,j}$ stops increasing because the next request to $p$ arrives, then $\bar{z}_{p,j}=0$ and $\tau^{\text{end}}=\tau(t(p,j+1)-1)$. Using Equation (\ref{eqn_y}), we get,
\[
\frac{1}{r}\cdot\left(\sum_{t=t(p,j)+1}^{t(p,j+1)-1}\bar{y}_t-\bar{z}_{p,j}\right)=\tau(t(p,j+1)-1)-\tau(t(p,j))=\tau^{\text{end}}-\tau(t(p,j))\text{.}
\]%\leq\frac{1}{s_{p,j}'}\ln\left(\frac{\bar{x}_{p,j}+1/k}{1/k}\right)\]
On the other hand, if $x_{p,j}$ stops increasing because it reaches $1$, then $z_{p,j}$ starts increasing from $0$ at the uniform rate $r$ at time $\tau^{\text{end}}$, and stops increasing at time $\tau(t(p,j+1)-1)$. Thus, $\bar{z}_{p,j}=r\cdot(\tau(t(p,j+1)-1)-\tau^{\text{end}})$. Again, using Equation (\ref{eqn_y}), we get,
\[
\frac{1}{r}\cdot\left(\sum_{t=t(p,j)+1}^{t(p,j+1)-1}\bar{y}_t-\bar{z}_{p,j}\right)=(\tau(t(p,j+1)-1)-\tau(t(p,j)))-(\tau(t(p,j+1)-1)-\tau^{\text{end}})=t^{\text{end}}-\tau(t(p,j))\text{.}
\]
Thus, in either case, we have,
\begin{equation}\label{eqn_yz}
\frac{1}{r}\cdot\left(\sum_{t=t(p,j)+1}^{t(p,j+1)-1}\bar{y}_t-\bar{z}_{p,j}\right)=\tau^{\text{end}}-\tau(t(p,j))\text{.}
\end{equation}

From Inequality (\ref{eqn_x}) and Equation (\ref{eqn_yz}), we get,
\[
\frac{1}{s_{p,j}'}\ln\left(\frac{\bar{x}_{p,j}+1/k}{1/k}\right)\geq\tau^{\text{end}}-\tau(t(p,j))=\frac{1}{r}\cdot\left(\sum_{t=t(p,j)+1}^{t(p,j+1)-1}\bar{y}_t-\bar{z}_{p,j}\right)\text{.}
\]
Rearranging, we get,
\[    \bar{x}_{p,j} \ge \frac1k \left(\exp \left(
        \frac{ s_{p,j}'}{r} \left( \sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t -
          \bar{z}_{p,j} \right) \right) - 1\right),
\]
as required.
\begin{comment}
We will show that the lemma holds for any $\tau$ and the corresponding $x_{p,j}(\tau)$, $y_t(\tau)$, $z_{p,j}(\tau)$ produced by the algorithm. Let
\[\tau_{p,j}' = \min \left(\{\tau > \tau(t(p,j)) \mid x_{p,j}(\tau) = 1\} \cup
\{\tau(t(p,j+1)-1)\} \right),
\] i.e., the smallest $\tau$ for which $x_{p,j}(\tau) = 1$ if it exists, or $\tau(t(p,j+1)-1)$ otherwise. This is the time $\tau$ after which $x_{p,j}$ stops increasing.

Let us fix $p$ and $j$ and consider the case $\tau < \tau_{p,j}'$. In this case, by the definition of the growth rates in the algorithm, we get the following differential equation if we consider $x_{p,j}(\tau)$ as a function of $y_t(\tau)$ for any $t$ such that $t(p,j)+1 \le t < t(p,j+1)$ and $\tau \le \tau_{p,j}'$, assuming for a moment that $s_{p,j}(\tau)$ is fixed:
\[ 
\frac{dx_{p,j}}{dy_t} = \frac{s_{p,j}(\tau)}{r} \left(x_{p,j} + \frac1k
\right).
\]

Taking $s_{p,j}'$ as above, we turn this into the inequality
\[
\frac{dx_{p,j}}{dy_t} \ge \frac{s_{p,j}'}{r} \left(x_{p,j} + \frac1k \right),
\] 
which we can solve using a standard separation of variables approach. Let $\tau''(t) = \min(\tau(t), \tau_{p,j}')$. Integrating over the interval $[\tau(t-1), \tau''(t)]$, which is the only interval during which both $y_t$ and $x_{p,j}$ can increase, gives
\begin{equation}\label{lem2basic} \ln\left(x_{p,j} + \frac1k \right)
\biggr\vert_{\tau(t-1)}^{\tau''(t)} \ge \frac{s_{p,j}'}{r} y_t
\biggr\vert_{\tau(t-1)}^{\tau''(t)}.
\end{equation} 
Expanding this expression gives
\[
\ln \left(x_{p,j}(\tau''(t)) + \frac1k \right) - \ln \left(x_{p,j}(\tau(t-1))
+ \frac1k \right) \ge \frac{s_{p,j}'}{r} (y_t(\tau''(t)) - y_t(\tau(t-1)),
\] 
which, using Observation \ref{o1}, gives
\[ 
\ln \left(x_{p,j}(\tau''(t)) + \frac1k \right) - \ln \left(x_{p,j}(\tau(t-1))
+ \frac1k \right) \ge \frac{s_{p,j}'}{r} y_t(\tau''(t)),
\] 
and we note that if $\tau(t) \ge \tau''(t)$ then $y_t(\tau(t)) = \bar{y}_t$, as it will no longer increase.

Summing over all rounds $t$ such that $t \ge t(p,j)+1$ and $\tau(t - 1) \le \tau_{p,j}'$, i.e., those during which $x_{p,j}$ is possibly increased and letting $t'$ denote the largest $t$ such that $\tau(t-1) \le \tau_{p,j}'$, gives
\[ 
\sum_{t = t(p,j)+1}^{t'} \left( \ln \left(x_{p,j}(\tau''(t)) + \frac1k
\right) - \ln \left(x_{p,j}(\tau(t-1)) + \frac1k \right) \right) \ge
\frac{s_{p,j}'}{r} \sum_{t = t(p,j)+1}^{t' - 1} \bar{y}_t + y_{t'}(\tau_{p,j}').
\] 
The left sum is telescoping, as for all $t < t'$ we have $\tau''(t) = \tau(t)$, and by Observation \ref{o2} we have $x_{p,j}(\tau(t(p,j)) = 0$.  Thus the above expression can be simplified to
\begin{equation*} \ln \left(x_{p,j}(\tau_{p,j}')) + \frac1k \right) - \ln \left(
\frac1k \right) \ge \frac{s_{p,j}'}{r} \sum_{t = t(p,j)+1}^{t' - 1} \bar{y}_t +
y_{t'}(\tau_{p,j}').
\end{equation*}

In the case $\tau_{p,j}' = \tau(t(p,j+1)-1)$ we are done, as $z_{p,j}$ is never increased and hence by taking exponentials and rearranging we obtain the statement of the lemma with $\bar{z}_{p,j} = 0$. Otherwise, we want to consider $\tau > \tau_{p,j}'$.  In this case we know that $x_{p,j}(\tau) = 1$ and the algorithm increases $z_{p,j}(\tau)$ rather than $x_{p,j}(\tau)$. This means the left hand side of Inequality \eqref{lem2basic} is no longer increasing while the right hand side term is still increasing.

For the inequality to continue to hold, we need to subtract $\frac{s_{p,j}'}{r} z_{p,j}(\tau)$ from the right hand side to counteract the increase of $y_t(\tau)$, yielding
\begin{equation}\label{lem2eq2} \ln \left(x_{p,j}(\tau) + \frac1k \right) - \ln
\left( \frac1k \right) \ge \frac{s_{p,j}'}{r} \left( \sum_{t = t(p,j) +
1}^{\hat{t} - 1} \bar{y}_t + y_{\hat{t}}(\tau) - z_{p,j}(\tau)\right).
\end{equation}

During a round $\hat t$ and time $\tau$ where $x_{p,j}(\tau) = 1$, $z_{p,j}(\tau)$ increases at rate $r$, which cancels out the increase of $y_{\hat t}(\tau)$, as the rate of change becomes
\[
\frac{d}{d\tau}\frac{s_{p,j}'}{r} \left( \sum_{t = t(p,j)+1}^{\hat{t} - 1}
\bar{y}_t + y_{\hat{t}}(\tau) - z_{p,j}(\tau)\right) = \frac{s_{p,j}'}{r} (r -
r) = 0.
\] 
Thus Inequality \eqref{lem2eq2} continues to hold as $\tau$ increases even while $x_{p,j}(\tau)$ remains constant at $1$.

The increase in $z_{p,j}(\tau)$ counteracts all increase in the right hand side from the time $\tau''(t')$, where $x_{p,j}(\tau)$ becomes $1$, until time $\tau(t(p,j+1)-1)$.  Afterwards, $z_{p,j}(\tau)$ will stay constant, so we have $\bar{z}_{p,j} = z_{p,j}(\tau(t(p,j+1)-1)$.

Finally, after examining the inequality for $\tau \ge \tau(t(p,j+1)-1)$ the expression becomes
\begin{equation*} \ln \left(k \bar{x}_{p,j} + 1 \right)\ge \frac{s_{p,j}'}{r}
\left( \sum_{t = t(p,j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \right),
\end{equation*} which gives the lemma after taking exponentials and rearranging.
\end{comment}
\end{proof}

\feasibility*
\begin{proof}
The first statement follows immediately from the definition of the algorithm and the fact that we can always fulfill the primal constraints, for example, by setting all the variables to $1$.

To show the second statement, we note that $\bar{x} \le \mathbf{1}$, which with Equation \eqref{lem2eq} gives us
\[ 
\frac1k \left(\exp \left( \frac{ s_{p,j}'}{r} \left( \sum_{t = t(p,
j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \right) \right) - 1\right) \le
\bar{x}_{p,j} \le 1.
\] 
Taking the left- and right-hand sides gives us, after rearranging and taking
logarithms,
\[
\sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \le
\frac{r}{s_{p,j}'} \ln(k + 1),
\] 
where the left hand side is $(A^T \bar{y} - \bar{z})_{p,j}$ as a $1$ only appears in the $(p,j)$th column of $A$ from row $t(p,j)+1$ through row $t(p,j+1)-1$.
\end{proof}

% \begin{proof}[Proof of Lemma~\ref{lem:inftytolog}] The first inequality is trivial. To obtain the second, note
% \[ \|x\|_{\log n}^{\log n} = \sum_{i = 1}^n |x_i|^{\log n} \le n \cdot \max_{i
% \in [n]}{|x_i|^{\log n}} = n \|x\|_\infty^{\log n}
% \] which, after taking roots gives the result, as $n^{\frac{1}{\log n}} = e$.
% \end{proof}

\roundinghelper*
\begin{proof}
  We define our rounded solution $x^{*}$ as
  \begin{equation*}
    x_{p,j}^{*} = \begin{cases} 0 & \text{if $x_{p,j} < \frac{1}{8k}$,} \\ \min\{\frac{1}{4k} \lceil 8k x_{p,j} \rceil, 1\} & \text{otherwise.} \end{cases}
  \end{equation*}
  That is, we round every variable $x_{p,j}$ of value less than $\frac{1}{8k}$ to $0$, and every variable of greater value will be doubled and then rounded up to the nearest multiple of $\frac{1}{4k}$.

  As each variable's value is at most doubled and then rounded up, the fractional cost for min-max paging can at most triple, as each variable in $x^{*}$ is no larger than $3$ times the corresponding variable in $x$ and the objective function $f(x)$ in min-max paging satisfies $f(cx) = cf(x)$ for any $c \in \mathbb{R}$. It remains to show that the solution $x^{*}$ is feasible.

  We note that the only variables whose value in $x^{*}$ can decrease during the rounding are those of value less than $\frac{1}{8k}$. The total number of such variables other than $p_{t}$ in a feasible solution is at most $k$, as otherwise.
  \[
    \sum_{B(t) \setminus \{p_{t}\}} x_{p,r(p,t)} \le n - 1 - k + \frac{1}{8k} k \le n-k.
  \]

  Hence we note that the total contribution $L$ of these variables to the constraint of round $t$ is at most $\frac{1}{8}$.

  As $n - k$ is an integer, and the fractional algorithm stops ejecting pages as soon as the constraint is satisfied, we know that $\sum_{p \in B(t) \setminus \{p_{t}\}} x_{p,r(p,t)}$ is integral.

  We further note that the contribution of all variables that are rounded up in this bound must therefore be at least $n - k - \frac18$

  If any variable $x_{p,j}$ in $x$ fulfills $\frac18 \le x_{p,j} \le \frac78$, then the rounding step will increase this variable by at least $\frac18$, which compensates the value lost by rounding down all small variables.

  Otherwise, if we let $A = \{x_{p,r(p,t)} \in B(t) \setminus \{p_{t}\} \mid x_{p,r(p,t)} \le \frac18 \}$ and $\sum_{x \in A} x \ge \frac18$, then the doubling of these variables compensates for the rounding down of small variables.

  Finally, if neither of these is the case, the variables of size greater than $\frac78$ must sum up to at most $n - k - L$, where $L$ denotes the amount of mass lost by rounding the small variables to $0$,  and at least $n - k - 2L > n - k - 1$. The sum of the rounded-up variables is an integer, as all variables of value greater than $\frac12$ are rounded to $1$, so we gain at least $L$ from rounding up the large variables.
\end{proof}


==> MinMax (Fair) Paging/app_randlb.tex <==
\subsection{Randomized Lower Bound: $k \ge 2$}
(Work in progress - Max)

\begin{thm}\label{thm_rlb}
  The randomized competitive ratio of min-max paging is
  $\Omega(\log(k+1) \log_{k+1} n) = \Omega(\log n)$, where $n$ is the number of
  pages and $k$ is the size of the cache.
\end{thm}

By Yao's principle, it suffices to exhibit a probability distribution on input
instances which forces every deterministic online algorithm to perform a factor
$\Omega(\log n)$ worse in expectation as compared to the optimum cost. Let
$n=(k+1)^m$ for some large integer $m$. Our randomized adversarial strategy
takes a parameter $N \gg n$ and is defined as follows.
\begin{algorithm}
  \caption{An adversarial input distribution for min-max paging}\label{adversary}
  \begin{algorithmic}
    \State Let $L_m=\{p^m_0,\ldots,p^m_{n-1}\}$ be a set of $n=(k+1)^m$ pages.
    \For{$\ell$ $=$ $m$ to $1$} \State $L_{\ell-1}\gets\emptyset$.  \For{$i$ $=$
      $0$ to $(k+1)^{\ell-1}-1$} \State Give $N$ requests, chosen uniformly and
    independently at random from the set of pages
    $p^{\ell}_{(k+1)i},p^{\ell}_{(k+1)i+1}, \dots, p^{\ell}_{(k+1)i+k}$.  \State
    $p^{\ell-1}_i$ $\gets$ a uniformly random page from
    $p^{\ell}_{(k+1)i},p^{\ell}_{(k+1)i+1}, \dots, p^{\ell}_{(k+1)i+k}$.  \State
    Add $p^{\ell-1}_i$ to $L_{\ell-1}$.  \EndFor \EndFor
  \end{algorithmic}
\end{algorithm}

We call each iteration of the outer for-loop a \textit{layer} and each of the
inner for-loop a \textit{phase}. We number layers $m,m-1,\ldots,1$.

Let $X_{i}^\ell$ be the number of faults incurred by page $p_i^\ell$ at the
beginning of layer $\ell$.

\begin{lem}
  For every layer $\ell$ and every $i \in \{0, (k+1)^\ell - 1\}$ we have
  $\mathbb{E}[X_i^\ell] \ge (m-l) \cdot N/(k+1)^2$.
\end{lem}
\begin{proof}
  We will prove this by reverse induction on the number of layers. We observe
  that $X_i^m = 0$ for all $i \in \{0, n-1\}$. Assume now that we have shown for
  each $i \in \{0, 1, \dots, (k+1)^\ell-1\}$ that
  $\mathbb{E}[X_i^\ell] \ge (m-\ell) \frac{N}{(k+1)^2}$. We will prove that for
  every $j \in \{0, 1, \dots, (k+1)^{\ell-1} - 1\}$ we have
  $\mathbb{E}[X_i^\ell] \ge (m-\ell+1) \frac{N}{(k+1)^2}$.

  During the $j$th phase of layer $\ell$ we give $N$ requests chosen uniformly
  at random from a set of $k+1$ pages. This means that any algorithm for min-max
  paging with a cache of size $k$ faults exactly when the page that is not in
  its cache at a given point in time is chosen for the next request. This
  happens with probability $\frac{1}{k+1}$ and so, by linearity of expectation,
  the algorithm will fault $\frac{N}{k}$ times in expectation. Let $Y_i^\ell$
  denote the number of page faults for a single page $p_i^\ell$ during the $j$th
  phase. At the end of the phase, we choose one of the pages uniformly at
  random, so the expected number of faults on this page, which will be
  $X_{j}^{\ell-1}$, becomes
  \begin{align*}
    \mathbb{E}[X_j^{\ell-1}] &\ge \sum_{i=0}^{k} \frac{1}{k+1} \mathbb{E}[X_{(k+1)j+i}^\ell] + \sum_{i=0}^{k} \frac{1}{k+1} \mathbb{E}[Y_i^\ell] \\
                             & = (m-\ell) \frac{N}{(k+1)^2} + \frac{N}{(k+1)^2} = (m - \ell + 1) \frac{N}{(k+1)^2}.
  \end{align*}
  The first term in the inequality is due to the induction hypothesis and the
  second term comes from the faults incurred during the current phase.
\end{proof}

By holding on to the page that will be moved on to the next layer and employing
the GreedyLFD strategy on the remaining $k$ pages with $k-1$ cache slots, we
find that OPT has cost $m + 4N / (k(k+1) H_{k+1})$.

\begin{lem}
  Assume $\sigma$ is a request sequence of length $T$ where each request is
  chosen uniformly at random from the set $p_1, p_2, \dots, p_{k+1}$. Then the
  cost of OPT for min-max paging on this request sequence is at most
  $4T / (k(k+1) H_{k+1})$.
\end{lem}
\begin{proof}
  We want to bound the expected number of requests needed to increase the cost
  of OPT, using the algorithm GreedyLFD. As in the deterministic case, we
  consider the variables $T_i$, which are now random variables, and denote the
  round during which $\max_{p \in P} \cost(GreedyLFD, \sigma, p, t)$ first
  reaches $i$.

  We note that $T_1 = 1$, as the algorithm GreedyLFD always starts with an empty
  cache. For $T_2$, we note that in expectation, it will be greater than
  $2 (k+1) H_{k+1}$, by the coupon collector's problem, as we need to request
  each page once to incur the first fault on each page, and subsequently, we
  need to request all pages again, before faulting for the second time on any
  page. This is because GreedyLFD, upon having seen all $k+1$ pages, will eject
  the page that comes last out of all of them, which next occurs after
  $(k+1) H_{k+1}$ time steps, in expectation.

  For general $i$, we will now show that
  $\mathbb{E}[T_{i+1}] \ge \frac{k(k+1}{4} (2H_{k+1} - 1) + E[T_{i}]$. Let us
  fix $i$ and assume we are currently at time $T_i$. That means there is one
  page of cost $i$ and all other pages are of cost less than $i$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm_rlb}]
  Take ratios between them
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/detlb.tex <==
%\subsection{Deterministic Lower Bound Idea}
%We first prove the following theorem.

\begin{lemma}
  Any deterministic algorithm $\ALG$ for min-max paging with cache size $k = 2$ is at least $\Omega(\log n)$-competitive.
\end{lemma}
\begin{proof}
  Suppose $n = 3^\ell$ and let the set of pages be $\{p_{1}, p_{2}, \dots, p_{n}\}$. We construct a bad request sequence $\sigma$ for $\ALG$ in $\ell$ layers. Each layer is further divided into phases. Let $N \gg n$ be a large integer parameter.

  We call the number of page faults incurred by page $p$ up to round $t$ the \emph{cost} of $p$ at $t$. Similarly, the \emph{cost of the min-max paging algorithm $\ALG$} is the maximum cost over all pages $p \in P$.

  % When we say \emph{cost of a page}, we mean the number of page faults after a request to that page, and similarly \emph{cost of an
  % algorithm} is its cost with respect to min-max paging that is maximum cost of a
  % page.

  We now iteratively construct the adversarial sequence $\sigma$, going layer by layer.

  Layer~1 will use all pages, that is the set $\{p_{1},p_{2}, \dots, p_{n}\}$.
\begin{itemize}
  \item In the first phase, we request pages $p_{1}$, $p_{2}$, and $p_{3}$ in such a way that $\ALG$ faults on every request, such a cruel sequence composed of $k+1$ pages exists for every deterministic algorithm for paging. We stop this phase once the cost of the algorithm becomes $N$, which must happen before sending $3N$ requests. Without loss of generality, we assume that the cost of $p_{1}$ first reaches $N$, and hence the costs of $p_{2}$ and $p_{3}$ are $< N$. These costs are the same as the number of requests to the respective pages because the algorithm always faults.

  \item In the second phase, we repeat this step with pages $p_{4}$, $p_{5}$, and $p_{6}$.
  Without loss of generality, we assume that the cost of $p_{4}$ is $N$.
  \item Repeat this process until the set of pages $\{p_{1}, p_{2}, \dots, p_{n}\}$ is exhausted.
\end{itemize}
In all phases, the adversary always keeps the lowest numbered page, that is pages $p_{1}, p_{4}, p_{7}, \ldots$, respectively, in the cache, incurring a cost of only $1$ on them, while the cost of the other pages is at most $N$.  We \emph{promote} pages $p_{1}, p_{4}, p_{7}, \ldots$ to Layer~2.

Layer~2 with universe of pages $\{p_{1}, p_{4}, p_{7}, ..., p_{n-2}\}$ is constructed exactly in the same way as Layer~1. After this layer, the cost of $\ALG$ is $2N$, whereas the cost of the adversary is $\le N$, with costs of pages $p_{1}, p_{10}, p_{19},\ldots$ having cost $\le 2$, and we \emph{promote} them to Layer~3, and so on.

After phase $i$, the number of pages in the universe becomes $n/3^i$, the cost of $\ALG$ becomes $iN$, whereas the adversary's cost is always $\le \max\{N, i\}$.  This gives us the desired lower bound using $\log_3(n)$ layers by choosing $N \ge \ell$.
\end{proof}

\paragraph{Generalizing the above construction} The idea behind the lower bound of $\Omega(k (\log n)/\log k)$ is as follows.  We generalize the construction above by using $n = (k+1)^\ell$ pages and $\ell = \log_{k+1}n$ layers. In each phase, we use $k{+}1$ pages and force the cost of the algorithm on one of these pages to increase by $N$.  The adversary's cost increases by at most $1$ on the page she will promote to the next layer. By using a smarter \emph{offline} algorithm, the cost of the adversary increases by at most $O(N/k)$ on the $k$ pages of this phase that will not be promoted. So, in the end, the adversary's cost is $O(\ell + N/k)$, whereas the cost of the algorithm is $\Omega(N\ell)$. We obtain the desired lower bound by choosing $N \ge c k \ell$ for a large enough constant $c$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/figure.tex <==
\begin{figure}
    \centering
    \[
    \begin{blockarray}{cccccccccccc}
     & \dots & x_{p_1,7} & x_{p_2,9} & x_{p_3, 3} & x_{p_1,8} & x_{p_4,5} & x_{p_2,10} & x_{p_5,3} & x_{p_1, 9} & \dots \\
    \begin{block}{c[ccccccccccc]}
    \vdots & \ddots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots &  \\
    t(p_1, 7) & \dots & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \dots \\
    t(p_2, 9) & \dots & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \dots \\
    t(p_3, 3) & \dots & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & \dots \\
    t(p_1, 8) & \dots & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & \dots \\
    t(p_4, 5) & \dots & 0 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & \dots \\
    t(p_2, 10) & \dots & 0 & 0 & 1 & 1 & 1 & 0 & 0 & 0 & \dots \\
    t(p_5, 3) & \dots & 0 & 0 & 1 & 1 & 1 & 1 & 0 & 0 & \dots \\
    t(p_1, 9) & \dots & 0 & 0 & 1 & 0 & 1 & 1 & 1 & 0 & \dots \\
    \myvdots & \dots & 0 & 0 & 1 & 0 & 1 & 1 & 1 & 1 & \dots \\
    \vdots &  & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots \\
    \end{block}
    \end{blockarray}\vspace*{-1.25\baselineskip}
    \]
    \caption{An example of the structure of a constraint matrix of the paging problem, corresponding to the sub-sequence of requests $p_1, p_2, p_3, p_1, p_4, p_2, p_5, p_1$ starting at time $t' = t(p_1, 7)$. The matrix is lower triangular, due to the columns being in order of the appearance of variables. In this example, we assume that the pages $p_1, p_2, p_3, p_4$ and $p_5$ have been requested $6, 8 , 2 , 4,$ and $2$ times before the appearance of this sequence respectively. }
    
%    \ac{Max, what are $j_1,\ldots, j_5$ here? Since this is an example anyways, you could take some concrete values of $j_p$'s and clarify in the caption that the subsequence appears right after $j_p$ requests to each page $p$ have been given.}
    \label{fig:matrix}
  \end{figure}

==> MinMax (Fair) Paging/fractional.tex <==
\section{A Fractional Algorithm for General Paging}

% 1. Defining properties of f
We study a general class of convex objective functions for the paging problem to arrive at a competitive algorithm for min-max paging. Let $x \in \mathbb{R}^{T}$ be the vector consisting of the variables $x_{p,j}$ in order of appearance in $\sigma$.
%
The objective functions $f: \mathbb{R}^{T} \to \mathbb{R}$ which we consider in this section have the following properties: (1) $f(0) = 0$; (2) $f(x)$ is a monotonically increasing function in $x$; (3) $\nabla f(x)$ is monotonically increasing in each coordinate; and (4) $f(x)$ has \emph{$q$-bounded growth}, i.e. there exists a positive integer $q$ such that for all $x \in \R_{+}^T$, $\langle \nabla f(x), x \rangle \le q f(x)$. In particular, any polynomial function of $x$ of degree $q$ will fulfill these requirements.

% 4. Monotonicity of Fenchel dual
% 5. Weak duality
% 6. Additional properties from abc+

%\subsection{Preliminaries}

% 2. Convex program
We formulate the general paging problem as an online convex program. Given a convex function $f: \R_{+}^n \to \R$ and a matrix $A \in \R^{m \times n}$, a general (offline) convex programming problem is to minimize $f(x)$ subject to $A x \ge \ones$ and $x \ge \zeros$.

In online convex programming, the rows of the constraint matrix $A$ are revealed one by one, corresponding to the request sequence $\sigma$. Upon receiving the $t$th row $A_{t}$ of the constraint matrix, the task of the algorithm is to increase the variables $x$ until the constraint $A_{t} x \ge 1$ is fulfilled. The algorithm is never allowed to decrease any of the variables in $x$.

In the fractional convex program for paging, we denote by $p_t$ the page requested in round $t$. Furthermore, we let $r(p,t)$ indicate the number of requests to page $p$ up to and including round $t$, and let $t(p,j)$ be the round during which the page $p$ is requested for the $j$'th time. As each round corresponds uniquely to a pair $(p,j)$, we have $\sum_{p} r(p,t) = T$.
We let $B(t) = \{p \in P | r(p,t) \ge 1 \}$ be the set of distinct pages encountered up to, and including, round $t$. The variables $x_{p,j}$ can now take values in the interval $[0,1]$ and indicate the fraction of the page the algorithm has removed from the cache between the $j$'th and $j+1$'st times it was requested.
%
Using this notation, the convex program for general paging looks as follows:
\begin{equation}\label{primal}
  \begin{array}{lll}
    \text{minimize} & f(x) \\ %= \sum_{p \in P} \left(w_p \sum_{j=1}^{r(p,T)} x_{p,j} \right)^q & \\
    \text{subject to} & \sum_{p \in P \setminus \{p_t\}} x_{p, r(p,t)} \ge |B(t)| - k & \forall t \in [T] \\
                    & 0 \le x_{p,j} \le 1 & \forall p \in [n], j \in [r(p,T)] \\
  \end{array}
\end{equation}
By using a convex objective function, this formulation generalizes prior work on online paging, including weighted paging \cite{bansalbn_12}.
%This primal uses the standard formulation for the constraints of a paging program due to \cite{bansalbn_12}, but it differs from all previous primals by the use of a convex objective function. 
Crucially, the box constraint $0 \le x_{p,j} \le 1$ means that the online convex programming framework of \cite{azarOnlineAlgorithms2016} can not be used to solve this program.

At the beginning of round $t$, we are given a new variable $x_{p_t,r(p_t,t)}$, which is initialized to $0$ along with the constraint $\sum_{p \in B(t) \setminus \{p_t\}} x_{p, r(p,t)} \ge |B(t)| - k$.  This constraint ensures that after each round $t$, at least $|B(t)|-k$ fractional page mass has been ejected, or, equivalently, at most $k$ fractional page mass is inside the cache.  We observe that the variable $x_{p,j}$ will only appear in the constraints corresponding to rounds $t \in \{t(p,j)+1, t(p,j)+2, \dots t(p,j+1)-1 \}$, i.e.~the variable $x_{p,j}$ does not appear in round $t(p,j)$ when it is requested. This is because we are not allowed to increase $x_{p,j}$ during this round, as page $p$ is required to be fully inside the cache in round $t(p,j)$, in order to serve the request.

% \subsection{Online Convex Programming}

% We will tackle the min-max paging problem via a convex objective, so set up some
% related preliminaries here.

% If $A$ has only non-negative entries, we call the problem a convex program with
% \emph{covering constraints}.  In online convex programming, we are given a
% vector of variables $x \in \mathbb{R}^n$, all of which are initialized to be
% zero, and the convex function $f(x)$.  The online request sequence corresponds
% to the rows of $A$.  In other words, the constraint matrix $A$ is revealed row
% by row.  Once a new constraint has been revealed, we have to increase $x$ until
% it is satisfied.  Then a new constraint is revealed, which must be satisfied by
% possibly increasing $x$, and so on.  We are not allowed to decrease variable
% $x_i$.

% %% TODO make a preliminary section on online algorithms where we can add this
% The quality of a solution to an online convex programming problem is measured
% by§ the \emph{competitive ratio}, which is the ratio between the optimal offline
% solution $\OPT$ and the solution $\ALG$ produced by an algorithm. In particular,
% if we let $\bar{x}$ be the vector $x$ produced by an online algorithm $\ALG$
% after having processed all $j$ rounds, then the competitive ratio is the minimum
% $r$ such that $f(\bar{x}) \le r \cost(\OPT)$.

% We will use the following lemma to reduce $\ell_\infty$-norm type cost to
% $\ell_{\log n}$-norm type cost.

% \begin{lem} For any vector $x \in \R^n$,
%   \[ \|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty.
% \]
% \label{lem:inftytolog}
% \end{lem}
% \begin{proof} The first inequality is trivial. To obtain the second, note
% \[ \|x\|_{\log n}^{\log n} = \sum_{i = 1}^n |x_i|^{\log n} \le n \cdot \max_{i
% \in [n]}{|x_i|^{\log n}} = n \|x\|_\infty^{\log n}
% \] which, after taking roots gives the result, as $n^{\frac{1}{\log n}} = e$.
% \end{proof}

% In this section we solve

% We consider a convex programming formulation of the paging problem: we replace
% the linear cost function $\sum_p w_p \sum_j x_{p,j}$ by a convex function $f(x)$
% which has the following properties:





% Our algorithm will use the relaxation of the above convex program where
% $x_{p,j} \in \{0, 1\}$ constraints are replaced by $0 \le x_{p,j} \le 1$
% constraints.  We recall that this represents a fractional version of the problem.

In order to define a dual for the convex program~\ref{primal}, we will need the following definition:

\begin{Definition}
Given a request sequence $\sigma$ of length $T$ consisting of pages from the set $P$, we can uniquely, up to relabeling of pages, define a constraint matrix $A
\in \{0,1\}^{T \times T}$ as
\[ %\text{\sag{Max, can you add a picture showing the matrix?} \mx{Added a drawing, let me know if it's alright or if i need to change it.}}
  A_{t,(p,j)} =
  \begin{cases} 1 & \text{if $t \in [t(p,j)+1, t(p,j+1) - 1]$}\\ 0 &
\text{otherwise.}
  \end{cases}
\]
In round $t$, we can determine all non-zero entries, as they only depend on the variables encountered up to round $t$.  Additionally, we can implicitly set the columns corresponding to future variables to $0$. If we order both the columns and rows by order of appearance, then the constraint matrix will be lower triangular, see Figure~\ref{fig:matrix} in the appendix.
\end{Definition}


  % 3. Fenchel dual
  \begin{Definition}
    Let $f: \mathbb{R}_{+}^{T} \to \mathbb{R}$ be a convex function. The fenchel dual $f^{*}: \mathbb{R}_{+}^{T} \to \mathbb{R}$ of $f$ is defined as $f^*(y) = \sup_{w \in \R_+^T} \left( \langle w, y \rangle - f(w) \right),$
%    \[
%      f^*(y) = \sup_{w \in \R_+^T} \left( \langle w, y \rangle - f(w) \right),
%    \]
    where $\langle w, y \rangle = \sum_{i=0}^T w_i \cdot y_i$ denotes the Euclidean scalar product.
  \end{Definition}

  We need the following property of the Fenchel dual in the analysis of our algorithm:

\begin{restatable}{property}{fenchelmonotone}
\label{o0} 
The Fenchel dual $f^*(y): \R_{+}^T \to \R$ of a convex function $f$ is monotonically increasing in $y$.
\end{restatable}


The dual will consist of two sets of $T$ variables each, denoted by $y_t$ and $z_{p,j}$, respectively.  We let $y$ be the vector consisting of the $y_t$ ordered increasingly in $t$ and $z$ being the vector consisting of the $z_{p,j}$ ordered the same way as $x$.

%The following will be our convex dual:
%\sag{Max, can you add references?  Where did we get the dual?  ABC+?  Where did they get it?} \mx{Added a reference to the Boyd book. }
We will use the following \emph{conjugate dual} $D(y,z)$ for our primal-dual algorithm. %(See~\cite{boyd2004convex}, Section 5.1.6 for details)
For the convex primal~\eqref{primal}, the conjugate dual is:
\begin{equation*}
  \begin{array}{ll}
    \text{maximize} & D(y,z) = \sum_{t=1}^T (|B(t)| - k) y_t -\sum_{p, j} z_{p,j} - f^*(A^\top y - z), \\
    \text{subject to} &
                        \begin{array}{ll}0 \le y_t & \forall t \in [T]\\
                          0 \le z_{p,j} & \forall p \in [n], j \in [r(p,T)]\,,\\
                        \end{array}
  \end{array}
\end{equation*}
% \sag{Ashish, enclose Fenchel dual in proper definition environment.} \ac{Definition of Fenchel dual, Observation~\ref{o0}, and Lemma~\ref{weakduality} must go to preliminaries or must be separated out as Section 4.1.}%

%\sag{Define $\langle w, y \rangle$.}
This dual differs from the dual used in \cite{bansalbn_12} by the inclusion of the Fenchel dual term $f^*(A^\top y - z)$ and from the dual used in \cite{azarOnlineAlgorithms2016} by the use of non-uniform coefficients for the $y_t$ variables and the inclusion of the variables $z_{p,j}$.
The dual will only be used to obtain a lower bound on $\OPT$ for the analysis of our algorithm, and it does not influence the primal solution the algorithm produces. It remains to show that the stated dual fulfills this property for the convex program~\eqref{primal}:

\begin{restatable}[Weak Duality]{lemma}{weakduality}
\label{weakduality}
  For any feasible $x \in [0,1]^T$ and $y, z \in \R_{+}^T$, we have
  \begin{equation*}
    f(x) \ge \sum_{t \in [T]} (|B(t)|-k) y_t - \sum_{p,j} z_{p,j} - f^*(A^\top y - z).
  \end{equation*}
\end{restatable}

% TODO add argument / link to paper

%\subsection{The Algorithm}




%\sag{I don't understand this sentence.}  It is not present in round
%  $t(p,j)$, as the invariant of the paging problem requires the page $p_t$ to be
%  fully inside the cache in the round during which it was requested.

% We now extend the convex programming framework of \cite{azarOnlineAlgorithms2016}, which did not allow upper bounds on the variables.  This leads to Algorithm \ref{fractional}.  

% The algorithm is based on a continuous time $\tau$ which initially is $0$ and increases throughout the algorithm's processing of the constraints.  As all variables start at $0$ when they are introduced and increase at a rate dependent on $\tau$, we can write $x_{p,j}(\tau)$, $y_t(\tau)$ and $z_{p,j}(\tau)$ to express the value of the variables as a function of $\tau$.

% Furthermore, we let $\tau(t)$ denote the value of $\tau$ after we finish processing the $t$th constraint.  Note that, by the algorithm $\tau(0) = 0$.

% The algorithm uses parameters $r$ and $s_{p,j}(\tau)$ which are to be determined later.  Note that $s_{p,j}(\tau)$ depends on the value of $\tau$, $p$ and $j$ and hence is not a constant parameter.

% \begin{algorithm}
%   \caption{A fractional algorithm for min-max paging}\label{fractional}
%   \begin{algorithmic}
%     \Require $r > 0$ and $s_{p, j}(\tau) > 0$, $s_{p,j}(\tau)$ monotonically decreasing in $\tau$
%     \State $\tau \gets 0$
%     \For{each round $t \in [T]$}
%     \State let $p_t$ be the page requested in this round
%     \State $x_{p_t,r(p,t)}(\tau) \gets 0$
%     \State $y_t(\tau) \gets 0$
%     \State $z_{p_t,r(p,t)}(\tau) \gets 0$
%     \While{$\sum_{p \in P \setminus \{p_t\}} x_{p,r(p,t)}(\tau) < |B(t)| - k$}
%     \State increase $\tau$ uniformly at rate $1$
%     \State increase $y_t(\tau)$ uniformly at rate $r$
%     \For{all $p \in P \setminus \{p_t\}$ in parallel}
%     \If{$x_{p,r(p,t)} < 1$}
%     \State increase $x_{p,r(p,t)}(\tau)$ at rate $s_{p,r(p,t)}(\tau) \left(x_{p, r(p,t)}(\tau) + \frac{1}{n}\right)$
%     \Else
%     \State increase the corresponding $z_{p, r(p,t)}(\tau)$ at rate $r$
%     \EndIf
%     \EndFor
%     \EndWhile
%     \EndFor
%   \end{algorithmic}
% \end{algorithm}

% \begin{obs}\label{o1}
%   We have $y_t(\tau(t-1)) = 0$ for all $t \in [T]$.
% \end{obs}
% \begin{proof}
%   By definition $\tau(t-1)$ is the time when we finish processing the $t-1$-st constraint, which equals the time when we start processing the $t$-th constraint, as $\tau$ is not increased between constraints.
%   By the algorithm, $y_t$ is initialized to $0$ at  time $\tau(t-1)$.
% \end{proof}
% % \begin{obs}\label{o2}
% %   We have $x_{p,j}(\tau(t(p,j))) = 0$ for all $p$ and $j$.
% % \end{obs}
% % \begin{proof}
% %   By the algorithm, $x_{p,j}$ is initialized to $0$ at the beginning of round $t(p,j)$ and is not increased until the next round which starts at time $\tau(t(p,j)+1)$, as invariant $1$ requires the page to be completely in the cache after processing this round, as we do not increase $\tau$ in between rounds.
% % \end{proof}

% \begin{lem}\label{xlowerbound}
%   Let  $\bar{x}$ denote the value of $x$ after processing the complete request sequence $\sigma$, similarly for $\bar{y}$ and $\bar{z}$.  If $s_{p,j}(\tau)$ is monotonically decreasing in $\tau$, then
%   \begin{equation}\label{lem2eq}
%     \bar{x}_{p,j} \ge \frac1n \left(\exp \left( \frac{ s_{p,j}'}{r} \left( \sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \right) \right)  - 1\right),
%   \end{equation}
%   where $s_{p,j}'$ is the minimum value that $s_{p,j}(\tau)$ takes on during the execution of the algorithm.%$ = s_{p,j}(\tau(t(p,j+1)-1))$.  %This is the minimal value that $s_{p,j}(\tau)$ takes on while $x_{p,j}(\tau)$ is being increased by our algorithm, as afterwards the variable corresponding to $p$ which increases is replaced by $x_{p,j+1}(\tau)$.\mh{we don't know yet how $s$ is defined so we don't understand this comment here.}
% \end{lem}
% \begin{proof}
%   We will show that the Lemma holds for any $\tau$ and the corresponding $x_{p,j}(\tau)$, $y_t(\tau)$, $z_{p,j}(\tau)$ produced by the algorithm.  Let 
%   \[\tau_{p,j}' = \min \left(\{\tau > \tau(t(p,j)) \mid x_{p,j}(\tau) = 1\} \cup \{\tau(t(p,j+1)-1)\} \right),
%   \]
%   i.e.  the smallest $\tau$ for which $x_{p,j}(\tau) = 1$ if it exists, or $\tau(t(p,j+1)-1)$ otherwise.  

%   Let us fix $p$ and $j$ and consider the case $\tau < \tau_{p,j}'$.  In this case, by the definition of the growth rates in the algorithm, we get the following differential equation if we consider $x_{p,j}(\tau)$ as a function of $y_t(\tau)$ for any $t$ such that $t(p,j)+1 \le t < t(p,j+1)$ and $\tau \le \tau_{p,j}'$, assuming for a moment that $s_{p,j}(\tau)$ is fixed:
%   \[
%     \frac{dx_{p,j}}{dy_t} = \frac{s_{p,j}(\tau)}{r} \left(x_{p,j} + \frac1n \right).
%   \]

%   Taking $s_{p,j}'$ as above, we turn this into the inequality
%   \[
%     \frac{dx_{p,j}}{dy_t} \ge \frac{s_{p,j}'}{r} \left(x_{p,j} + \frac1n \right),
%   \]
%   which we can solve using a standard separation of variables approach.  Let $\tau''(t) = \min(\tau(t), \tau_{p,j}')$.  Integrating over the interval $[\tau(t-1), \tau''(t)]$, which is the only interval during which both $y_t$ and $x_{p,j}$ can increase, gives 
%   \begin{equation}\label{lem2basic}
%     \ln\left(x_{p,j} + \frac1n \right) \biggr\vert_{\tau(t-1)}^{\tau''(t)} \ge \frac{s_{p,j}'}{r} y_t \biggr\vert_{\tau(t-1)}^{\tau''(t)}.
%   \end{equation}
%   Expanding this expression gives
%   \[
%     \ln \left(x_{p,j}(\tau''(t)) + \frac1n \right) - 
%     \ln \left(x_{p,j}(\tau(t-1)) + \frac1n \right) \ge \frac{s_{p,j}'}{r} (y_t(\tau''(t)) - y_t(\tau(t-1)),
%   \]
%   which, using Observation \ref{o1}, gives 
%   \[
%     \ln \left(x_{p,j}(\tau''(t)) + \frac1n \right) - 
%     \ln \left(x_{p,j}(\tau(t-1)) + \frac1n \right) \ge \frac{s_{p,j}'}{r} y_t(\tau''(t)),
%   \]
%   and we note that if $\tau(t) \ge \tau''(t)$ then $y_t(\tau(t)) = \bar{y}_t$, as it will no longer increase.

%   Summing over all rounds $t$ such that $t \ge t(p,j)+1$ and $\tau(t - 1) \le \tau_{p,j}'$, i.e.  those during which $x_{p,j}$ is possibly increased and letting $t'$ denote the largest $t$ such that $\tau(t-1) \le \tau_{p,j}'$, gives
%   \[
%     \sum_{t = t(p,j)+1}^{t'} \left( \ln \left(x_{p,j}(\tau''(t)) + \frac1n \right) - \ln \left(x_{p,j}(\tau(t-1)) + \frac1n \right) \right) \ge \frac{s_{p,j}'}{r} \sum_{t = t(p,j)+1}^{t' - 1} \bar{y}_t + y_{t'}(\tau_{p,j}').
%   \]
%   The left sum is telescoping, as for all $t < t'$ we have $\tau''(t) = \tau(t)$, and %by Observation \ref{o2} 
%   we have $x_{p,j}(\tau(t(p,j)) = 0$.  Thus the above expression can be simplified to
%   \begin{equation*}
%     \ln \left(x_{p,j}(\tau_{p,j}')) + \frac1n \right) - \ln \left( \frac1n \right) \ge \frac{s_{p,j}'}{r} \sum_{t = t(p,j)+1}^{t' - 1} \bar{y}_t + y_{t'}(\tau_{p,j}').
%   \end{equation*}

%   In the case $\tau_{p,j}' = \tau(t(p,j+1)-1)$ we are done, as $z_{p,j}$ is never increased and hence by taking exponentials and rearranging we obtain the statement of the lemma with $\bar{z}_{p,j} = 0$.  Otherwise, we want to consider $\tau > \tau_{p,j}'$.  In this case we know that $x_{p,j}(\tau) = 1$ and the algorithm increases $z_{p,j}(\tau)$ rather than $x_{p,j}(\tau)$.  This means the left hand side of Inequality \eqref{lem2basic} is no longer increasing while the right hand side term is still increasing.  

%   In order for the inequality to continue to hold, we subtract $\frac{s_{p,j}'}{r} z_{p,j}(\tau)$ from the right hand side in order to counteract the increase of $y_t(\tau)$, yielding 
%   \begin{equation}\label{lem2eq2}
%     \ln \left(x_{p,j}(\tau) + \frac1n \right) - \ln \left( \frac1n \right) \ge \frac{s_{p,j}'}{r} \left( \sum_{t = t(p,j) + 1}^{\hat{t} - 1} \bar{y}_t + y_{\hat{t}}(\tau) - z_{p,j}(\tau)\right).
%   \end{equation}

%   During a round $\hat t$ and time $\tau$ where $x_{p,j}(\tau) = 1$, $z_{p,j}(\tau)$ increases at rate $r$, which cancels out the increase of $y_{\hat t}(\tau)$, as the rate of change, i.e.  the derivative, becomes
%   \[
%     \frac{d}{d\tau}\frac{s_{p,j}'}{r} \left( \sum_{t = 1}^{\hat{t} - 1} \bar{y}_t + y_{\hat{t}}(\tau) - z_{p,j}(\tau)\right) = \frac{s_{p,j}'}{r} (r - r) = 0.
%   \]
%   Thus Inequality \eqref{lem2eq2} continues to hold as $\tau$ increases even while $x_{p,j}(\tau)$ remains constant at $1$.

%   The increase in $z_{p,j}(\tau)$ counteracts all increase in the right hand side from the time $\tau''(t')$, where $x_{p,j}(\tau)$ becomes $1$, until time $\tau(t(p,j+1)-1)$ whence $z_{p,j}(\tau)$ will stay constant, thus we have $\bar{z}_{p,j} = z_{p,j}(\tau(t(p,j+1)-1)$.

%   Finally, after examining the inequality for $\tau \ge \tau(t(p,j+1)-1)$ the expression becomes 
%   \begin{equation*}
%     \ln \left(n \bar{x}_{p,j} + 1 \right)\ge \frac{s_{p,j}'}{r} \left( \sum_{t = t(p,j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \right),
%   \end{equation*}
%   which gives the lemma after taking exponentials and rearranging.
% \end{proof}

% This immediately implies the following:

% \begin{claim}\label{feasibility1}
%   The $x(\tau(t))$ produced by Algorithm \ref{fractional} throughout its execution are feasible for the primal for all $t \in [T]$ and the vector $(A^\top \bar{y} - \bar{z})_{p,j} \le \frac{r}{s_{p,j}'} \ln(n+1)$.
% \end{claim}
% \begin{proof}
%   The first statement follows via the definition of the algorithm immediately from the fact that we can always fulfill the primal constraints, for example by setting all the variables to $1$.

%   To show the second statement, we note that $\bar{x} \le \mathbf{1}$, which with Equation \eqref{lem2eq} gives us
%   \[
%     \frac1n \left(\exp \left( \frac{ s_{p,j}'}{r} \left( \sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j} \right) \right)  - 1\right) \le \bar{x}_{p,j} \le 1.
%   \]
%   Taking the left- and right-hand sides, after rearranging and taking logarithms gives us
%   \[
%     \sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t - \bar{z}_{p,j}  \le \frac{r}{s_{p,j}'} \ln(n + 1),
%   \]
%   where the left hand side is $(A^T \bar{y} - \bar{z})_{p,j}$ as a $1$ only appears in the $(p,j)$th column of $A$ from row $t(p,j)+1$ through row $t(p,j+1)-1$.
% \end{proof}

% \begin{obs}
%   The function $s_{p,j}(\tau) = \frac{\partial f(x(\tau))}{\partial x_{p,j}}^{-1}$ is monotonically decreasing in $\tau$.
% \end{obs}
% \begin{proof}
%   This immediately follows from the fact that we require the gradient to be non-decreasing in each coordinate.
% \end{proof}
% % \begin{proof}
% %   We claim that the gradient of a convex function is monotonically increasing in each $x_{p,j}(\tau)$.  Once this is established, the observation follows immediately from the definition of $s_{p,j}(\tau)$.
% %   
% %   Now, by the definition of a convex, differentiable function $g(w)$ we have
% %   \[
% %     g(w) \ge g(z) + \langle \nabla g(z), w - z \rangle,
% %   \]
% %   for any vectors $w$ and $z$ in its domain.  Hence, we also have 
% %   \[
% %     g(z) \ge g(w) + \langle \nabla g(w), z - w \rangle,
% %   \]
% %   and by adding the two inequalities, we get
% %   \begin{equation}\label{o7}
% %     0 \le \langle \nabla g(w) - \nabla g(z), w - z \rangle.
% %   \end{equation}
% %   
% %   Now consider vectors $y$ and $y'$ where $y' = y + c \cdot e_m$, where $e_m$ is the $m$th standard basis vector and $c > 0$ is a constant.  Using Inequality \eqref{o7} we find that $0 \le \langle \nabla g(y') - \nabla g(y), c \cdot e_m \rangle$, which gives $\frac{\partial g} {\partial y_m}(y) \le \frac{\partial g}{\partial y_m}(y')$ by the fact that $c > 0$.  As $m$ was arbitrary, the claim follows.
% % \end{proof}

% For the final theorem we need to define $q$, the \emph{polynomial growth} of a function, which is defined as the smallest integer such that for all $x \in \R_{\ge 0}^T$,
% \[
%   \langle \nabla f(x), x \rangle \le q f(x).
% \]

% \begin{thm}\label{thm:frac}
%   After processing the sequence $\sigma$, Algorithm \ref{fractional} produces an $O((k q \log(n+1))^q)$ competitive solution $\bar{x}$ for fractional min-max paging with an objective function that has polynomial growth $q$, if we set $s_{p,j}(\tau) = \frac{\partial f(x)}{\partial x_{p,j}}^{-1}$ and $r = \frac{\delta}{\ln(n+1)}$ where $\delta$ will be determined in the proof.
% \end{thm}
% \begin{proof}
%   By weak duality, it suffices to show that the primal is no larger than $O((k q \log n)^q)$ times the dual which is a lower bound on OPT by weak duality.

%   We will now bound the growth rates of the primal and dual for each round $t$ in terms of $\tau$.  It suffices to only consider the case $A_t x(\tau) < |B(t)| - k$, as otherwise nothing needs to be done.

%   Let \[C_t(\tau) = \{ (p,j) \mid t(p,j) < t < t(p,j+1) \text{ and } x_{p,j}(\tau) < 1 \}\] be the set of indices of variables $x_{p,j}(\tau)$ at round $t$ which correspond to a page that is (partially) in the cache, i.e.  the indices of the variables corresponding to the last request of a given $p$, which are increasing and have not been fully removed from the cache.  

%   Similarly, let 
%   \[
%     D_t(\tau) = \{ (p,j) \mid t(p,j) < t < t(p,j+1) \text{ and } x_{p,j}(\tau) = 1 \}
%   \]
%   be the set of indices of the variables $x_{p,j}(\tau)$ which have been fully removed from the cache since their previous request and which correspond to the last request to a given page $p$.  Note that $|C_t(\tau)| + |D_t(\tau)| = |B(t)| - 1$, as they include a variable for each page except the page $p_t$.

%   While processing the $t$-th constraint, we have, by the choice of $s_{p,j}(\tau)$, and the fact that $x_{p,j}(\tau)$ is constant if $(p,j) \in D_t(\tau)$:
%   \begin{align*}
      %       G_1 \coloneqq \frac{df(x)}{d\tau} = \sum_{p,j} \frac{\partial f(x)}{\partial x_{p,j}} \frac{\partial x_{p,j}(\tau)}{\partial \tau}  &= \sum_{p,j} \frac{\partial f(x)}{\partial x_{p,j}} \left( s_{p,j}(\tau) \left(x_{p,j}(\tau) + \frac1n \right) \right) \\
%     &= \sum_{i \in C_t{(\tau)}} \left(x_{p,j}(\tau) + \frac1n \right) \le |C_t(\tau)| + 1.
% \end{align*}
% The first equality is due to the chain rule for vector-valued functions, while the last inequality follows as there are no more than $n$ pages in $C_t(\tau)$ at any time, hence the second term in the summation sums to at most $1$ and each $x_{p,j}(\tau) \le 1$.

% For the linear term $\sum_{t} (|B(t)|-k)y_t(\tau) - \sum_{p,j} z_{p,j}(\tau)$ in the dual, we find that, in round $t$, as $y_t$ may only increase during that round, and the fact that both $\frac{dy_t(\tau)}{d\tau} = r$ and $\frac{dz_{p,j}(\tau)}{d\tau} = r$ if $(p,j) \in D_t(\tau)$,
% \begin{align*}
% G_2 \coloneqq \frac{d \sum_{t} (|B(t)|-k)y_t(\tau) - \sum_{p,j} z_{p,j}(\tau)}{d\tau} = (|B(t)| - k) r - \sum_{(p,j) \in D_t(\tau)} r = r (|B(t)| - k - |D_t(\tau)|).
% \end{align*}

% The ratio $\frac{|B(t)| - k - |D_t(\tau)|}{|C_t(\tau)|+1} = \frac{|C_t(\tau)| - k + 1}{|C_t(\tau)|+1} = 1 - \frac{k-1}{|C_t(\tau)|+1}$ is minimized when $|C_t(\tau)| = k$, as  (1) it is monotonically increasing in $|C_t(\tau)|$ and (2) $|C_t(\tau)| > k - 1$, since otherwise all but $k$ pages (the $k-1$ pages of $C_t(\tau)$ and the page requested at time $t$)  have been ejected, which means the constraint $A_t x(\tau) \ge |B(t)|-k$ must be satisfied.  Thus the minimum of $\frac{|B(t)| - k - |D_t(\tau)|}{|C_t(\tau)|+1}$  is $\frac{1}{k+1}$ and the ratio between the growth rates of the primal and the linear term of the dual is bounded from below by 
% \[
% \frac{G_2}{G_1} \ge \frac{r}{k+1}.
% \]
% As both functions start from $0$ at time $\tau = 0$, their values after processing all elements are also bounded by this ratio as our primal never grows faster than the linear term times this ratio.  Thus with our choice of $r$ it follows that 
% \[
% \sum_t (n-k) \bar{y}_t - \sum_{p,j} \bar{z}_{p,j} \ge
% \frac{\delta}{(k+1)\ln(n+1)} f(\bar x)
% \]
% %Finally, from the fact that $x_{p,j} \le 1$ we get that 
% %\[
% %\frac1n \left(\exp \left( \frac{ s_{p}'}{r} \left( \sum_{t = t(p, j)+1}^{t(p,j+1)-1} y_t - z_{p,j} \right) %\right)  - 1\right) \le 1,
% %\]
% %which, after rearranging yields
% %\[
% %\sum_{t = t(p, j)+1}^{t(p,j+1)-1} y_t - z_{p,j} \le r \frac{\partial f(\bar x)}{\partial x_{p,j}} \ln(n + 1).
% %\]
% %The choice for $s_p'$ is justified as $\nabla f(x)$ is monotonically increasing, since $f(x)$ is convex.
% % clear up this sentence
% Plugging 
% $s_{p,j}(\tau) = \frac{\partial f(x)}{\partial x_{p,j}}^{-1}$ and $r = \frac{\delta}{\ln(n+1)}$ 
% %our choice of $s_{p,j}(\tau)$ and $r$ 
% into the second statement of Claim \ref{feasibility1}, we obtain that $A^T y - z \le \delta \nabla f(\bar{x})$, which allows us to bound the conjugate term of the dual as
% \[
% f^*(A^T \bar y - \bar z) \le f^*(\delta \nabla f(\bar x)) \le 
% \begin{cases}
% \delta^{\frac{q}{q-1}} \cdot (q - 1) \cdot f(\bar x) & \text{ if $q > 1$},\\
% 0 & \text{ if $q = 1$},
% \end{cases}
% \]
% where the second inequality uses Lemma 4 of \cite{azarOnlineAlgorithms2016} and the first inequality is due to Observation \ref{o0}.
% Hence the relationship between the final value $D(\bar y, \bar z)$ of the dual and the final value $f(\bar x)$ of the primal is
% \[
% D(\bar y, \bar z) = \sum_t (n-k) \bar{y}_t - \sum_{p,j} \bar{z}_{p,j} - f^*(A^T \bar y - \bar z) \ge 
% \left( \frac{\delta}{(k+1) \ln(1+n)} - \delta^{\frac{q}{q-1}} \cdot (q - 1)\right) \cdot f(\bar x).
% \]
% The term $\left( \frac{\delta}{(k+1) \ln(1+n)} - \delta^{\frac{q}{q-1}} \cdot (q - 1)\right)$ is a polynomial in $\delta$.  It is maximized for $\delta = \frac{1}{((k+1) \ln(n + 1) q)^{q-1}}$ giving a competitive ratio of $\frac{1}{((k+1) q \ln(n+1))^q}$,  which is positive for $n\ge 2$.  Hence, by rearranging and weak duality we obtain 
% \[
% f(\bar{x}) \le \left((k+1) q \ln(n+1) \right)^q D(\bar y, \bar z) \le \left((k+1) q \ln(n+1) \right)^q f(\OPT).
% \]
% \end{proof}

% To obtain the cost vector $\mathbf{c}(t)$, we sum the costs $x_{p,j}(\tau(t))$ for each page $p$.  We define a matrix $C \in \{0,1\}^{n \times T}$ such that the $p$-th row of $C$ contains a $1$ in column $(p,j)$ for each of the variables $x_{p,j}$ for $j \in [r(p,T)]$ and $0$ otherwise.
% It follows that $C \cdot x(\tau(t)) = \mathbf{c}(t)$ for all $t \in [T]$.  Note that the solution of the fractional min-max paging problem could be determined by setting $f(x)$ to $\|C x \|_\infty$.

% However note that $\|\cdot \|_\infty$ is not differentiable and, thus, we cannot apply the above directly to 
% $\|C x \|_\infty$.  Thus, instead we run the above algorithm with
% $f(x) :=\|C x \|_{\log n}^{\log{n}}.$ 
% This is a polynomial in the variables of $x$ with maximum degree $\log n$, hence $q = \log n$.  We further note that the gradient of this function is monotonous in the sense that for any $x'$ and $x$ where $x'$ is pointwise greater than $x$ we have $\nabla f(x') > \nabla f(x)$ pointwise as well.

% Note that $\|C x \|_{\log n}^{\log n}$ produces an $n$-approximation of
% $\|C x \|_\infty^{\log n}$ as shown by the next lemma, which states a well-known fact about  norms in finite-dimensional vector spaces.

% 
% \begin{lem}
% For any vector $x \in \R^n$,
% \[
% \|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty.
% \]
% \end{lem}
% \begin{proof}
% The first inequality is trivial.  To obtain the second, note
% \[
% \|x\|_{\log n}^{\log n} = \sum_{i = 1}^n |x_i|^{\log n} \le n \cdot \max_{i \in [n]}{|x_i|^{\log n}} = n \|x\|_\infty^{\log n}
% \]
% which, after taking roots gives the result, as $n^{\frac{1}{\log n}} = e$.
% \end{proof}
% Let $x^*$ denote the optimum solution for the problem with $\ell_{\infty}$-norm.  
% Thus, from Theorem~\ref{thm:frac} it follows that
% $$\| x^*\|_{\infty}^{\log n} \le \| x^*\|_{\log n}^{\log n} 
% \le \| {\bar x}\|_{\infty}^{\log n} = P(\bar x) 
% \le (( k+1) \log^2 (n +1))^{\log n} \| x^*\|_{\log n}^{\log n} \le n (( k+1) \log^2 (n +1))^{\log n} \| x^*\|_{\infty}^{\log n}.$$
% Applying the $\log n$-th root shows that $P(\bar x)^{1/\log n}$ gives an 
% $O(k \log^2 n)$-approximation to the optimum solution.
%  
% %  (Note that $\|Cx\|_{\log n}^m$ is not differentiable at $0$ for any $m < \log n$, so we can not simply choose $m = O(1)$ to remove a $\log$-factor, unless we are fine without differentiability at $0$ (probably the case))

% Note that the gradient of $\|Bx\|_{\log n}^{\log n}$ is $0$ at $0$, so we start the algorithm at $\epsilon \mathbf{1}$ for a small $\epsilon > 0$ instead, which incurs at most an additive cost of $\epsilon$.

% \begin{cor}
% There exists a $O(k \log^2 n)$ competitive algorithm for fractional min-max paging.
% \end{cor}

% \section{Improving the Competitive Ratio}

% To improve on the competitive ratio, one promising direction is to use $\|Bx\|_p$, the $\ell_p$-norm instead of its $p$th power as the target function.

% It is easy to see that this function fulfills the following properties from
% Remark 1:
% \begin{itemize}
%     \item Convexity, by the triangle inequality: $\|B(1-\alpha)x + B\alpha y\|_p \le (1-\alpha)\|Bx\|_p + \alpha \|By\|_p$.
%     \item Monotonicity, trivially as it is a norm.
%     \item $\|B \mathbf{0}\|_p = 0$.
%     \item Differentiability everywhere but $0$.
% \end{itemize}

%However, it lacks the following

%\begin{itemize}
%    \item Pointwise monotonicity of the gradient
%\end{itemize}

%We notice that the function $\|Bx\|_p$ is not differentiable at the point
% $\mathbf{0}$.  If we instead start the algorithm at a suitably small $\epsilon$
% step away from the origin, we incur no more than an additive error and the
% rest of the analysis goes through as we do not rely on the differentiability
% of a given point when we are not in said point.  As
% $\langle \nabla \|Bx\|_p, x \rangle = \|Bx\|_p$ we have the following:

% We extend the convex programming framework of
% \cite{azarOnlineAlgorithms2016}, which does not allow upper bounds on the
% variables.  
Our online algorithm, given in Algorithm \ref{fractional} uses a continuous time $\tau$, which is 0 initially and increases throughout the algorithm. Let $\tau(t)$ denote the value of $\tau$ when we finish processing the $t$'th constraint and let $\tau(0) = 0$. As all variables are $0$ at creation and increase at a rate dependent on $\tau$, we use $x_{p,j}(\tau)$, $y_t(\tau)$, $z_{p,j}(\tau)$ to denote the values of the variables $x_{p,j}$, $y_t$, $z_{p,j}$ respectively at time $\tau$. Let $t(\tau)$ be the unique $t$ such that $\tau\in[\tau(t-1),\tau(t))$.
%\end{defn}
%\sag{Max, for each $t \in [T]$, define a semi-open interval of $\tau$.}
%
The algorithm uses parameters $r$ and $s_{p,j}(\tau)$ fixed later.  Note that $s_{p,j}(\tau)$ depends on the value of $\tau$, $p$ and $j$ and, thus, is not a constant parameter.

Our algorithm maintains dual variables $y$ and $z$ such that $A^\top y - z \le \delta \nabla f(x)$ is approximately fulfilled,~i.e.~, $A^\top y - z \le r \delta \nabla f(x)$ for some constant $r \ge 1$, which will then appear in the competitive ratio.  
%This approach is fundamentally similar to the primal-dual algorithms used for linear programming and, in the case of a linear target function, is equivalent to maintaining an \emph{approximately feasible dual}.  
We observe that if $f(x) = c^\top x$, the gradient is $c$ and we get $A^\top y - z \le c$, which is the dual constraint in the linear program for weighted paging. The reason why this point-wise upper bound is necessary is because, together with Property~\ref{o0}, it allows us to upper-bound the convex conjugate term $f^*(A^\top y - z)$ in $D(y,z)$ in terms of the primal function $f(x)$.  For general $w$ the conjugate $f^*(w)$ may be arbitrarily large as it is a convex function in $w$.


\begin{algorithm}
  \caption{A fractional algorithm for min-max paging}\label{fractional}
  \begin{algorithmic}[1]
    \Require $r > 0$ and $s_{p, j}(\tau) > 0$, $s_{p,j}(\tau)$ monotonically decreasing in $\tau$ 
    \State $\tau \gets 0$

    \For{each round $t \in [T]$}

    \State let $p_t$ be the page requested in this round 
    \State $x_{p_t,r(p,t)}(\tau) \gets 0$, $y_t(\tau) \gets 0$, $z_{p_t,r(p,t)}(\tau) \gets 0$

    %\While{$\sum_{p \in B(t) \setminus \{p_t\}} x_{p,r(p,t)}(\tau) < |B(t)| -  k$}

    \State{$\frac{d y_{t}(\tau)}{d\tau} \gets r$}

    \State{$\frac{d x_{p,r(p,t)}(\tau)}{d\tau} \gets \begin{cases} s_{p,r(p,t)}(\tau) \left(x_{p,r(p,t)}(\tau) + \frac{1}{k} \right) & \text{if } x_{{p,r(p,t)}}(\tau) < 1 \\ 0 & \text{otherwise} \end{cases}$}

    \State{$\frac{d z_{p,r(p,t)}(\tau)}{d\tau} \gets \begin{cases} r & \text{if } x_{{p,r(p,t)}}(\tau) = 1 \\ 0 & \text{otherwise} \end{cases}$}

    \State{Increase $\tau$, $y_{t}(\tau)$, $x_{p,r(p,t)}(\tau)$ and $z_{p,r(p,t)}(\tau)$ for all $p \in B(t) \setminus \{p_{t}\}$ simultaneously as per the above differential equations until $\sum_{p \in B(t) \setminus \{p_t\}} x_{p,r(p,t)}(\tau) \ge |B(t)| - k$}

    % \State increase $\tau$ uniformly at rate $1$

    % \State increase $y_t(\tau)$ uniformly at rate $r$

    % \For{all $p \in B(t) \setminus \{p_t\}$ in parallel}

    % \If{$x_{p,r(p,t)} < 1$}

    % \State increase $x_{p,r(p,t)}(\tau)$ at rate
    % $s_{p,r(p,t)}(\tau) \left(x_{p, r(p,t)}(\tau) + \frac{1}{k}\right)$

    % \Else \State increase the corresponding $z_{p, r(p,t)}(\tau)$ at rate $r$

    % \EndIf

    % \EndFor

    % \EndWhile

    \EndFor
\end{algorithmic}
\end{algorithm}

% \begin{observation}\label{o1} We have $y_t(\tau(t-1)) = 0$ for all $t \in [T]$ and the function $s_{p,j}(\tau) = \frac{\partial f(x(\tau))}{\partial x_{p,j}}^{-1}$ is monotonically decreasing in $\tau$.
% \end{observation}
% \begin{proof} 
% By definition, $\tau(t-1)$ is the time when we finish processing the $t-1$-st constraint, which equals the time when we start processing the $t$-th constraint, as $\tau$ is not increased between constraints. By the algorithm, $y_t$ is initialized to $0$ at time $\tau(t-1)$.
%\end{proof}

%\begin{obs}\label{o2}
%  We have $x_{p,j}(\tau(t(p,j))) = 0$ for all $p$ and $j$.
% \end{obs}
%\begin{proof}
%  By the algorithm, $x_{p,j}$ is initialized to $0$ at the beginning of round
%  $t(p,j)$ and is not increased until the next round which starts at time
%  $\tau(t(p,j)+1)$, as invariant $1$ requires the page to be completely in the
%  cache after processing this round, as we do not increase $\tau$ in between
%  rounds.
%\end{proof}

Next, to bound the conjugate term in the dual, it is necessary to obtain a bound on the dual ``constraints" $A^\top y - z$, which we obtain by relating the constant growth of $y_t$ and $z_{p,j}$ to the exponential growth of the $x_{p,j}$:
%due to the choice of growth rates:

\begin{restatable}{lemma}{xlowerbound}
  \label{xlowerbound} 
  Let $\bar{x}$ denote the value of $x$ after processing the complete request sequence $\sigma$, and similarly for $\bar{y}$ and $\bar{z}$.  If $s_{p,j}(\tau)$ is monotonically decreasing in $\tau$, then
  \begin{equation}
    \label{lem2eq}
    \bar{x}_{p,j} \ge \frac1k \left(\exp \left(
        \frac{ s_{p,j}'}{r} \left( \sum_{t = t(p, j)+1}^{t(p,j+1)-1} \bar{y}_t -
          \bar{z}_{p,j} \right) \right) - 1\right),
  \end{equation}
  where $s_{p,j}'$ is the minimum value that $s_{p,j}(\tau)$ takes on during the execution of the algorithm.
  % $ = s_{p,j}(\tau(t(p,j+1)-1))$.
  % This is the minimal value that %$s_{p,j}(\tau)$ takes on while $x_{p,j}(\tau)$ is
  % being increased by %our algorithm, as afterwards the variable corresponding to
  % $p$ which increases is replaced by $x_{p,j+1}(\tau)$.\mh{we don't know yet how
  % $s$ is defined so we don't understand this comment here.}
\end{restatable}

The following is an immediate consequence of the previous lemma and the fact that $x_{p,j} \le 1$:

\begin{restatable}{lemma}{feasibility}
    
\label{feasibility1}
The $x(\tau(t))$ produced by Algorithm \ref{fractional} throughout its execution are feasible for the primal for all $t \in [T]$ and the vector $(A^\top \bar{y} - \bar{z})_{p,j} \le \frac{r}{s_{p,j}'} \ln(k+1)$.
\end{restatable}

%OMIT FOR CONFERENCE SUBMISSION
%\begin{proof} This immediately follows from the fact that $f(x)$ is a polynomial
%of degree $q$ with positive coefficients.
%\end{proof}
%\begin{proof}
%  We claim that the gradient of a convex function is monotonically increasing
%  in each $x_{p,j}(\tau)$.  Once this is established, the observation follows
%  immediately from the definition of $s_{p,j}(\tau)$.
%
%  Now, by the definition of a convex, differentiable function $g(w)$ we have
%\[
%  g(w) \ge g(z) + \langle \nabla g(z), w - z \rangle,
%\]
%for any vectors $w$ and $z$ in its domain.  Hence, we also have
%\[
%  g(z) \ge g(w) + \langle \nabla g(w), z - w \rangle,
%\]
%and by adding the two inequalities, we get
%\begin{equation}\label{o7}
%0 \le \langle \nabla g(w) - \nabla g(z), w - z \rangle.
%\end{equation}
%
%Now consider vectors $y$ and $y'$ where $y' = y + c \cdot e_m$, where $e_m$ is
% the $m$th standard basis vector and $c > 0$ is a constant.  Using Inequality
% \eqref{o7} we find that
% $0 \le \langle \nabla g(y') - \nabla g(y), c \cdot e_m \rangle$, which gives
% $\frac{\partial g} {\partial y_m}(y) \le \frac{\partial g}{\partial y_m}(y')$
% by the fact that $c > 0$.  As $m$ was arbitrary, the claim follows.
%\end{proof}


The conjugate of a convex function with bounded growth can be bounded in terms of the original function and $q$, using the following lemma:

\begin{lemma}[\cite{azarOnlineAlgorithms2016}]\label{conjugateabc}
Let $f: \mathbb{R}_{\ge 0}^T \to \mathbb{R}_{\ge 0}$ be a monotone, convex, differentiable function satisfying $f(0) = 0$.  If there is a $q > 1$ such that $\langle \nabla f(x), x \rangle \le q f(x)$, then for any $0 < \gamma < 1$, $y \in \mathbb{R}_{\ge 0}^T$, $f^*(\gamma y) \le \gamma^{\frac{q}{q-1}} \cdot f^*(y)$ and $f^*(\gamma \nabla f(y)) \le \gamma^{\frac{q}{q-1}} (q-1) f(y)$.
%the following statements hold.
%\begin{enumerate}
 %  \item For $\delta \ge 1$, and any $x \in \mathbb{R}_{\ge 0}^T$, $f(\delta x) \le \delta^q f(x)$.
 %   \item For all $x \in \mathbb{R}_{\ge 0}^T$, $f^*(\nabla f(x)) \le (q-1) \cdot f(x)$.
%    \item If $q > 1$, then for any $0 < \gamma < 1$, $y \in \mathbb{R}_{\ge 0}^T$, $f^*(\gamma y) \le \gamma^{\frac{q}{q-1}} \cdot f^*(y)$ and $f^*(\gamma \nabla f(y)) \le \gamma^{\frac{q}{q-1}} (q-1) f(y)$.
   % \item If $q = 1$, then for any $0 < \gamma < 1$, $y \in \mathbb{R}_{\ge 0}^T$, $f^*(\gamma \nabla f(y)) \le 0$.
%\end{enumerate}
\end{lemma}

\begin{theorem}\label{thm:frac}
  %\sag{Max, add a reference to the convex program and Algo.  Maybe add the properties $f$ here instead of Remark~1.}
  Let $f(x)$ be a convex function satisfying the requirements stated at the beginning of this section, and let $\sigma$ be any request sequence. If we set $s_{p,j}(\tau) = \frac{\partial f(x)}{\partial x_{p,j}}^{-1}$ and $r = \frac{1}{\ln(k+1)(2q\ln(k+1))^{q-1}}$, then Algorithm~\ref{fractional} produces a $(2q \log(k+1))^q$-competitive solution $\bar{x}$ for fractional paging with objective function $f(x)$ in an online manner.
    
  %Then, after processing the request sequence
  %$\sigma$, Algorithm \ref{fractional} produces an $O((q \log(k+1))^q)$
%  competitive solution $\bar{x}$ for fractional $q$-paging, if we set
%  $s_{p,j}(\tau) = \frac{\partial f(x)}{\partial x_{p,j}}^{-1}$ and
%  $r = 1/((\ln(k+1)(2 q \ln(k + 1) )^{q-1})$. 
%\sag{Max, get rid of $\delta$ from the proof.  Remember: $\delta = 1/(2 q \ln(k + 1) )^{q-1}$.  Suggestion from Ashish, keep $r$ as the only parameter and minimize competitive ratio wrt $r$ to find value of $r$.}
\end{theorem}
\begin{proof}
  By weak duality, it suffices to show that the primal is no larger than $O((q \log(k+1))^q)$ times the dual, which is a lower bound on the cost of an optimal solution $x^*$ by weak duality.
%
  We will bound the primal and the dual growth rates for each round $t$. It suffices to only consider the case $A_t x(\tau) < |B(t)| - k$, as otherwise, the round is finished, and nothing needs to be done. 
  
  The processing of round $t$ begins at time $\tau(t - 1)$ and will last until $\tau(t)$, so we assume that $\tau \in (\tau(t-1), \tau(t)]$ for the remainder of this proof.
%
%\sag{Max, once you add definition of $t(\tau)$, the subscripts $t$ can go away.} \mx{I don't see how it would make it nicer since we need to reference $\tau$ twice in that case. You'd still need to refer to $\tau$ for the $t(\tau)$ interval and the actual time, as the set of variables that are equal to $1$ can change during the interval.}
  Let $C_t(\tau) = \{ (p,j) \mid t(p,j) < t < t(p,j+1) \text{ and } x_{p,j}(\tau) < 1 \}$ be the set of indices of variables $x_{p,j}(\tau)$ in round $t$ which correspond to a page that is (partially) in the cache, i.e., the indices of the variables corresponding to the latest request of a given $p$, which are increasing and have not been fully removed from the cache.
%
  Similarly, let $D_t(\tau) = \{ (p,j) \mid t(p,j) < t < t(p,j+1) \text{ and } x_{p,j}(\tau) = 1 \}$ be the set of indices of the variables $x_{p,j}(\tau)$ which have been fully removed from the cache since they have been last requested and which correspond to the latest request to a given page $p$.  Note that $|C_t(\tau)| + |D_t(\tau)| = |B(t)| - 1$, as the sets $C_t(\tau)$ and $D_t(\tau)$ are disjoint and include a variable for each page except the page $p_t$.
%
While processing the $t$-th constraint, we have, by the choice of $s_{p,j}(\tau)$, and the fact that $x_{p,j}(\tau)$ is constant if $(p,j) \in D_t(\tau)$:
  \begin{align}\label{g1}
    G_1 \coloneqq \frac{df(x)}{d\tau} = \sum_{p,j} \frac{\partial f(x)}{\partial x_{p,j}} \frac{\partial x_{p,j}(\tau)}{\partial \tau}
    &=\sum_{(p,j) \in C_t{(\tau)}} \frac{\partial f(x)}{\partial x_{p,j}} \left( s_{p,j}(\tau) \left(x_{p,j}(\tau) + \frac1k \right) \right) \\
    &= \sum_{(p,j) \in C_t{(\tau)}} \left(x_{p,j}(\tau) + \frac1k \right) \le |B(t)| - k - |D_t(\tau)| + \frac{|C_t(\tau)|}{k}.\label{eq7}
  \end{align}
  The first equality is due to the chain rule for vector-valued functions. The second equality uses the definition of $\frac{\partial x_{p,j}(\tau)}{\partial \tau}$ and the fact that $x_{p,j}$ does not change for $(p,j) \notin C_t{(\tau)}$.  And, the last inequality follows from the fact that the variables in $D_t(\tau)$ are all equal to $1$.
  %the primal constraint corresponding to round $t$,
  %\[ \sum_{p \in B(t) \setminus \{p_t\}} x_{p,r(p,t)}(\tau) < |B(t)| - k, \] can be rewritten as
  %\[ \sum_{p \in C_t(\tau)} x_{p,r(p,t)}(\tau) < |B(t)| - k - |D_t(\tau)|, \] as 
  

Note that only the $y_t$ corresponding to round $t$ may increase during round $t$. For the linear term $\sum_{t} (|B(t)|-k)y_t(\tau) - \sum_{p,j} z_{p,j}(\tau)$ in the dual, it holds that in round $t$
  %the fact that both $\frac{dy_t(\tau)}{d\tau} = r$ and
  %$\frac{dz_{p,j}(\tau)}{d\tau} = r$ if $(p,j) \in D_t(\tau)$
  \begin{align}\label{g2} 
  G_2 \coloneqq \frac{d}{d\tau} \left( \sum_{t} (|B(t)|-k)y_t(\tau) - \sum_{p,j}
    z_{p,j}(\tau) \right) = (|B(t)| - k) r - \sum_{(p,j) \in D_t(\tau)} r = r
    (|B(t)| - k - |D_t(\tau)|).
  \end{align}
  
We note that the right-hand side of Equation~\eqref{g2} is $r$-times the first term of the right-hand side of Equation~\eqref{eq7}.
%
%  We further note that this gives, together with Equation~\eqref{g1}, %\sag{Max, can you add an equation number to
%    definition of $G_1$ and refer it here?}
%  $G_1 \le \frac{1}{r} G_2 + \frac{|C_t(\tau)|}{k}$. 
Furthermore, 
%the term $\frac{|C_t(\tau)|}{k}$ can be bounded as
$\frac{|C_t(\tau)|}{k} \le |C_t(\tau)| - k + 1 = |B(t)| - 1 - |D_t(\tau)| - k + 1 = \frac1r G_2,$ since $|C_t(\tau)| \ge k$. %\sag{Max, this is not true.  Ashish and I believe
%    that the RHS of this inequality is just $k$, not $k+1$, and you need to
%    appropriately update the argument above.}
%
By adding together Equation~\eqref{g2} and the last inequality, we obtain
\begin{equation}\label{eq11}
G_1 \le |B(t)| - k  - |D_t(\tau)| + |C_t(\tau)|/k \le G_2/r  + G_2/r = 2 G_2/r.
\end{equation}


%  Thus we get $G_1 \le \frac2r G_2$.  \sag{Max, how do we get this?  It is clear
%    to us, but certainly not clear to the reader.}

Since both the primal and the linear term of the dual initially have value $0$ at time $\tau = 0$, their overall competitive ratio after processing all elements will be $\frac2r$. %values after
%  processing all elements remain bounded by this ratio as our primal never grows
%  faster than the linear term times this ratio (\sag{Max, which ratio?}).  
  Thus for the choice of $r(\delta) = \frac{\delta}{\ln(k+1)}$, where $\delta$ is a parameter which we will optimize later,
  %(\sag{Max, which choice?} \mx{Made more explicit})
  from Equation~\eqref{eq11} it follows that $\sum_t (B(t)-k) \bar{y}_t - \sum_{p,j} \bar{z}_{p,j} \ge \frac{\delta}{2\ln(k+1)} f(\bar x).$
  % Finally, from the fact that $x_{p,j} \le 1$ we get that
  % \[
  %   \frac1n \left(\exp \left( \frac{ s_{p}'}{r} \left( \sum_{t = t(p,
  %         j)+1}^{t(p,j+1)-1} y_t - z_{p,j} \right) %\right) - 1\right) \le 1,
  %     \]
  %     which, after rearranging yields
  %     \[
  %       \sum_{t = t(p, j)+1}^{t(p,j+1)-1} y_t - z_{p,j} \le r \frac{\partial f(\bar
  %       x)}{\partial x_{p,j}} \ln(n + 1).
  %     \]
  %     The choice for $s_p'$ is justified as $\nabla f(x)$ is monotonically
  %     increasing, since $f(x)$ is convex.   clear up this sentence
  Plugging $s_{p,j}(\tau) = \frac{\partial f(x)}{\partial x_{p,j}}^{-1}$ and
  $r(\delta) = \frac{\delta}{\ln(k+1)}$ into the second statement of Claim \ref{feasibility1}, we obtain that $A^T y - z \le \delta \nabla f(\bar{x})$, which allows us to bound the conjugate term of the dual as
  \[
    f^*(A^T \bar y - \bar z) \le f^*(\delta \nabla f(\bar x)) \le 
    \begin{cases}
      \delta^{\frac{q}{q-1}} \cdot (q - 1) \cdot f(\bar x) & \text{ if $q > 1$},\\
      0 & \text{ if $q = 1$},
    \end{cases}
  \]
  %\sag{Max, why are you giving reasoning for the second inequality first?  Also,
 %   you copied Lemma~4 for ABC+ into our paper earlier.  Why are you not
 %   referring to that?}
 where the first inequality is due to Property~\ref{o0} and the second inequality uses Lemma~\ref{conjugateabc}.  Hence the relationship between the final value $D(\bar y, \bar z)$ of the dual and the final value $f(\bar x)$ of the primal is

  % \sag{Max, why $B(t)$ instead of $n$?  $D(y,z)$ is not defined this way.} Max: Changed n to |B(t)|
  
  \[
    D(\bar y, \bar z) = \sum_t (|B(t)|-k) \bar{y}_t - \sum_{p,j} \bar{z}_{p,j} -
    f^*(A^T \bar y - \bar z) \ge \left( \frac{\delta}{2 \ln(1+k)} -
      \delta^{\frac{q}{q-1}} \cdot (q - 1)\right) \cdot f(\bar x).
  \]
  The term $h(\delta) = \left( \frac{\delta}{2 \ln(k+1)} - \delta^{\frac{q}{q-1}} \cdot (q - 1)\right)$ is a polynomial in $\delta$, which governs our competitive ratio. The best competitive ratio is obtained if we find $\delta \in (0,1)$ such that $h(\delta)$ is maximized. We find a local maximum at $\delta^* = \frac{1}{(2 q \ln(k + 1) )^{q-1}}$, yielding $h(\delta^*) = \frac{1}{(2 q\ln(k+1))^q}$.  By rearranging and weak duality (Lemma~\ref{weakduality}) we obtain
  \[
    f(\bar{x}) \le \left(2 q \ln(k+1) \right)^q D(\bar y, \bar z) \le \left(2 q \ln(k+1) \right)^q f(x^*),
  \]
  where $x^*$ is an optimal solution.
\end{proof}


%  \sag{Max, the way you have written makes it seem like $q$-norm satisfies
%    properties in Remark~1.  But it does not.  So please prove the following
%    theorem properly with inequalities and everything.}

%  In particular, for the function $f$, chosen at the beginning of this section,
%  after taking roots, we get the following theorem:

%Theorem~\ref{thm:frac} can be applied to the $q$th power the $\ell_q$-norm, which is a polynomial function in $x$ of degree $q$ and therefore satisfies the assumptions of Remark~1. 

The $\ell_q$-norm does not lie in our class of objective functions, as a coordinate of $\nabla f(x)$ can decrease while we increase all coordinates of $x$, hence we can not apply Theorem~\ref{thm:frac} straight away.
%obtain an $O(q \log(k+1))$-competitive solution:

\begin{theorem}\label{qpaging}
Let $q \in [1, \infty)$.  Then there exists a $2q \log(k+1)$-competitive algorithm for fractional $q$-paging with a cache of size $k$.
\end{theorem}
\begin{proof}
Let us fix $q \in [1, \infty)$. We apply Theorem~\ref{thm:frac} with the target function $f(x) = \sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} x_{p,j}\right)^q$, which is the $q$th power of the $\ell_q$-norm. This produces a solution $\bar{x}$, which is $(2q \log(k+1))^q$-competitive for the paging problem with target function $f(x)$.

Let $g: \mathbb{R} \to \mathbb{R}$ be a monotone function, then a solution $x$ to the paging problem with target function $f(x)$ will also be a feasible solution to the paging problem with target function $g(f(x))$. In particular, as $g$ preserves the standard ordering on the reals, an optimal solution to paging with target function $f(x)$ will remain an optimal solution to the problem with target function $g(f(x))$.

If we let $g(y) = y^{\frac{1}{q}}$ and we let $x^*$ be an optimal solution to the paging problem with target function $f(x)$, then $g(f(x))$ will be the $\ell_q$-norm and we find that $g(f(\bar{x})) \le g((2q \log(k+1))^q f(x^*)) = 2q \log(k+1) g(f(x^*))$.
\end{proof}

\begin{Remark} 
Note that if the gradient of $f(x)$ is $0$ at $x=0$, then we start the algorithm at $\epsilon \cdot \mathbf{1}$ for a small $\epsilon > 0$ instead, which can be chosen sufficiently small, so it does not influence the competitive ratio.
\end{Remark}

%\subsection{An Upper Bound for Min-Max Paging}

%Min-max paging is the case of $\infty$-paging, but find that the $\ell_\infty$-norm is not
%differentiable. However, using the following lemma on the constants in the equivalence of norms, we find that the $\ell_\infty$-norm of a vector lies within a constant
%factor of the vector's $\ell_{\log n}$-norm.


% \begin{lem} 
% \label{lem:inftytolog}
% For any vector $x \in \R^n$, $\|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty$.
% \end{lem}

We use
Theorem~\ref{qpaging} to show that we can obtain a $2e\log(n) \log(k+1)$-competitive fractional solution for $\infty$-paging by reducing it to $\log n$-paging.

\begin{theorem}\label{thm_frac_ub}
  There exists a $2e \log(n) \log(k+1)$-competitive algorithm for fractional
  min-max paging.
\end{theorem}

% We will use the following lemma to reduce $\ell_\infty$-norm cost to
% $\ell_{\log n}$-norm cost.

% To obtain the cost vector $\mathbf{c}(t)$, we sum the costs $x_{p,j}(\tau(t))$
% for each page $p$.  We define a matrix $C \in \{0,1\}^{n \times T}$ such that
% the $p$-th row of $C$ contains a $1$ in column $(p,j)$ for each of the
% variables $x_{p,j}$ for $j \in [r(p,T)]$ and $0$ otherwise.   It follows that
% $C \cdot x(\tau(t)) = \mathbf{c}(t)$ for all $t \in [T]$.  Note that the
% solution of the fractional min-max paging problem could be determined by setting
% $f(x)$ to $\|C x \|_\infty$.

% However note that $\|\cdot \|_\infty$ is not differentiable and, thus, we
% cannot apply the above directly to $\|C x \|_\infty$.  Thus, instead we run the
% above algorithm with $f(x) :=\|C x \|_{\log n}^{\log{n}}.$
\begin{proof}
Let $x^*$ be the optimal solution to the $\infty$-paging problem for the request sequence $\sigma$. We denote the cost of this solution by $\OPT_\infty$. 
%Lemma~\ref{lem:inftytolog} guarantees us that the solution $x^*$ yields a solution of cost no more than $e \cdot \OPT_\infty$ for $\log n$-paging.
%
Let $\bar{x}$ denote the fractional solution obtained using Algorithm~\ref{fractional}. By Theorem~\ref{qpaging} and $\|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty$, we know that this solution has cost
\[
\max_{p \in P} \sum_{j=1}^{r(p,T)} \bar{x}_{p,j} \le \left(\sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} \bar{x}_{p,j} \right)^{\log n} \right)^{\frac{1}{\log n}} \le 2 \log(n) \log(k+1) \cdot \OPT_{\log n} \le 2e \log(n) \log(k+1) \cdot \OPT_{\infty},
\]
where $\OPT_{\log n}$ denotes the cost of an optimal solution to the $\log n$-paging problem with input $\sigma$.
%
%$ and the second inequality follows from the fact that $\|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty$.%
%
% Finally, %by Lemma~\ref{lem:inftytolog},
% %as $\|x\|_\infty \le \|x\|_{\log n} \le e \|x\|_\infty$
% it follows that
% %\[
% $\max_{p \in P} \sum_{j=1}^{r(p,T)} \bar{x}_{p,j} \le \left(\sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} \bar{x}_{p,j} \right)^{\log n} \right)^{\frac{1}{\log n}},$
% %\]
This implies  that $\bar{x}$ is a $2e \log(n) \log(k+1)$-competitive solution for $\infty$-paging.
%This yields the following theorem:
\end{proof}

% Note that $\|C x \|_{\log n}^{\log n}$ produces an $n$-approximation of
% $\|C x \|_\infty^{\log n}$ as shown by Lemma~\ref{lem:inftytolog}.

% Let $x^*$ denote an optimal solution for $\infty$-paging and let
% $\bar{x}$ denote a solution produced by our algorithm for $\log n$-paging. 

% If the solution $x^*$ has cost $\OPT_infty$ for $\infty$-paging, then, by Lemma~1, there exists a solution
% for $\log n$-paging of cost no greater than $n^{\frac{1}{\log n}} \OPT_\infty = e \cdot \OPT_\infty$. The solution $\bar{x}$ produced by our algorithm will be no greater than $4 \log(n) \log(k+1) \cdot \OPT_{\log n}$, and in particular, $4e \log(n) \log(k+1) \cdot \OPT_\infty$.

% 

% 

% From
% Theorem~\ref{thm:frac} it follows that
% \begin{align*}
% \max_{p \in P} \sum_{j=1}^{r(p,T)} x_{p,j}^* 
% &\le \left( \sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} x_{p,j}^* \right)^{\log n} \right)^{\frac{1}{\log n}} \\
% &\le \left( \sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} \bar{x}_{p,j} \right)^{\log n} \right)^{\frac{1}{\log n}} \\
% &\le O(\log n \log k) \left( \sum_{p \in P} \left(\sum_{j=1}^{r(p,T)} x_{p,j}^* \right)^{\log n} \right)^{\frac{1}{\log n}}\\ 
% &\le O(\log n \log k) \max_{p \in P} \sum_{j=1}^{r(p,T)} x_{p,j}^*.
% \end{align*} 
% % (Note that $\|Cx\|_{\log n}^m$ is not differentiable at $0$ for any
% % $m < \log n$, so we can not simply choose $m = O(1)$ to remove a
% % $\log$-factor, unless we are fine without differentiability at $0$ (probably
% % the case))
% \sag{Max, the above chain of inequalities actually does not show what we need.
%   Please fix and write a correct proof.  Also please add a concrete competitive
%   ratio without big-O notation.}  This yields the following theorem for
% fractional min-max paging:


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/header.tex <==
% Language setting
% Replace `english' with e.g. `spanish' to change the document language
\usepackage[english]{babel}

% Set page size and margins
% Replace `letterpaper' with `a4paper' for UK/EU standard size
%\usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}
\usepackage[margin=1in]{geometry}

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}

\usepackage[T1]{fontenc}
\usepackage{kpfonts}%  for math    
\usepackage{libertine}%  serif and sans serif
\usepackage[scaled=0.85]{beramono}%% mono

% Useful packages
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage[colorlinks=true, allcolors=blue]{hyperref}
\usepackage{algorithm}
\usepackage{algpseudocodex}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{mathtools}
\usepackage{verbatim}

\usepackage{mdframed}

\usepackage{wrapfig}
\newcommand{\erclogowrapped}[1]{%
\setlength\intextsep{0pt}%
\begin{wrapfigure}[3]{r}{#1*\real{1.1}}%
\includegraphics[width=#1]{LOGO_ERC-FLAG_EU_crop.jpg}%
\end{wrapfigure}%
}

% for drawing the constraint matrix
\usepackage{blkarray, bigstrut}
% used to have vdots without bad spacing
\makeatletter
\DeclareRobustCommand
  \myvdots{\vbox{\baselineskip4\p@ \lineskiplimit\z@
    \hbox{.}\hbox{.}\hbox{.}}}
\makeatother

\makeatletter
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

%\usepackage{lineno}
%\linenumbers

\theoremstyle{plain}
\declaretheorem{theorem}
\declaretheorem[sibling=theorem]{claim}
\declaretheorem[sibling=theorem]{lemma}
\declaretheorem[sibling=theorem]{corollary}
\declaretheorem[sibling=theorem]{observation}
\declaretheorem[sibling=theorem]{property}
\theoremstyle{definition}
\declaretheorem[sibling=theorem]{Definition}
\declaretheorem[sibling=theorem]{assumption}
\declaretheorem[sibling=theorem]{Remark}


% declarewtheorem{theorem}{Theorem}
%\newtheorem{thm}{Theorem}
%\newtheorem{claim}[thm]{Claim}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{obs}[thm]{Observation}
%\theoremstyle{definition}
%\newtheorem{defn}[thm]{Definition}
% \newtheorem{assumption}[thm]{Assumption}
%\newtheorem{rem}[thm]{Remark}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\zeros}{\mathbf{0}}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\ALG}{\mathrm{ALG}}
\DeclareMathOperator{\cost}{cost}
\DeclareMathOperator{\len}{len}
\DeclareMathOperator{\poly}{poly}

\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}


\newcommand{\mh}[1]{\textit{\textcolor{blue}{MH: #1}}}
\newcommand{\sag}[1]{\textit{\textcolor{red}{Sagar: #1}}}
\newcommand{\mx}[1]{\textit{\textcolor{purple}{Max: #1}}}
\newcommand{\ac}[1]{\textit{\textcolor{magenta}{Ashish: #1}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Paging problem: intro and motivation from operating systems

Paging is a decades-old, classical computer science problem. Suppose a computer process working on $n$ \emph{pages} of data has access to two levels of memory: a fast memory, called the \emph{cache}, that can hold a small amount $k$ of pages, and a slow memory containing all $n$ pages. Typically, $k$ is much smaller than $n$, and initially, all pages are in slow memory. Whenever the process accesses a page, it is read from the cache; if it is not already in the cache, a \emph{page fault} occurs, and the page must be brought into the cache, which possibly necessitates \emph{evicting} another page from the cache to make room. This is called \emph{serving} the request. In the \emph{online} setting, each request must be served before the algorithm sees the subsequent request. The goal is to minimize the \emph{total number of page faults} incurred while serving a sequence of requests.

The paging problem has found new applications in communication networks, where caching is ubiquitous and is used to minimize energy usage, communication latency, and network traffic.  %albeit with a different goal, i.e.~function to minimize. 
Consider, for example, TCP connections that are kept alive on a router~\cite{cohen1999connection} or optical links in reconfigurable data center topologies~\cite{foerster2019survey, bienkowski2021online}. Every user application prefers to have an active connection, as re-establishing a TCP connection or link takes time and slows down communication or computation. Another example is content on web pages that is cached in a content delivery network, such as Akamai. In practice, the cache servers in these networks rely on dynamic, eviction-based algorithms for managing cache contents that solve the so-called content placement problem~\cite{thomdapu2021dynamic}. Web pages in the cache have a clear advantage as they can be served faster to the user than web pages that must be re-fetched from the server. 
Ideally, all applications (of the same priority) and all web pages should be treated equally.
This motivates us to propose the study of a \emph{fair} variant of paging, which we call \textit{min-max paging}. Its goal is to minimize the number of page faults on \emph{any} page, i.e.~to minimize the \emph{maximum number of page faults of any single page}.


% Paging as an online problem, definition of online algorithms and competitive
% ratio

In the \emph{online} setting, the page requests are revealed one by one without  knowledge of the future, so the description of how to serve each request must depend only on the request sequence thus far and the current cache contents. Naturally, for many problems, an online algorithm cannot output an optimal solution to a given instance -- something an {\em offline} algorithm having access to the entire input can produce. The sub-optimality of an online algorithm is usually measured using competitive analysis. Informally, we say that an online algorithm has a competitive ratio of $c$ if, on every problem instance, it produces a solution with (expected) cost at most $c$ times the cost of an optimal solution.
For the classic online paging problem the competitive ratio has been well-studied: It is $O(k)$ for deterministic algorithms~\cite{SleatorT85,karlinMRS86}
 and $H_k \approx 0.577 + \ln(k)$ for randomized algorithms~\cite{FiatKLMSY_JAlg91,10.1007/BF01759073}.
\begin{comment}
Sleator and Tarjan~\cite{sleaterT85} gave a tight bound of $k$ for the online paging. A well-known class of algorithms called \emph{marking} algorithms are $k$-competitive~\cite{karlinMRS86}. In the case of randomized algorithms, we assume that the adversary is oblivious to the random bits used by the algorithm. Fiat et al.~\cite{FIAT1991685} gave the first bounds for randomized algorithms: an upper bound of $2H_k$ and a lower bound of $H_k$, where
$H_k = 1 + 1/2 + 1/3 + \cdots + 1/k \approx 0.577 + \ln(k)$ is the $k$'th harmonic number. McGeoch and Sleator~\cite{10.1007/BF01759073} closed the gap showing an upper bound of $H_k$.
\end{comment}
%\ac{I prefer to have only an informal definition here, and move the following formal definition to the preliminaries section. Given such an online algorithm $A$, we define the \emph{cost} $c_A(\sigma)$ of the algorithm $A$ as the number of page faults when using $A$ on the request sequence $\sigma$.  (The algorithm $A$ still sees requests from $\sigma$ one-by-one.)  By $c^*(\sigma)$, we denote the minimum number of page faults achievable by any offline algorithm.  Then, we say that the competitive ratio $A$ is $C$ or that $A$ is $C$-competitive if for any $n$ and $k$
%\begin{equation}
%  \label{eq:defcr}
%  \text{there exists } b \text{ such that for all request sequences } \sigma:  c_A(\sigma) \le C \cdot c^*(\sigma) + b\,;
%\end{equation}
%we note that $b$ can depend on $n$ and $k$.  This is the complexity measure of interest throughout the paper, so whenever we talk about ``bounds,'' we are talking about bounds on competitive ratio.
%%%  ALTERNATIVE SIMPLER DEFINITION %%%
% Then the competitive ratio $A$ is defined as
% \begin{equation}
%   \label{eq:defcr}
%   \sup_\sigma \frac{c_A(\sigma)}{c^*(\sigma)}\,.
% \end{equation}
% If $A$ has competitive ratio $C$, we also say that $A$ is $C$-competitive.
%}


% Motivation for min-max paging, a semi-formal definition, previous (closely
% related) works, if any


% (Possibly semi-formal) statements of our results in theorem environment
%
To the best of our knowledge, the min-max paging problem has not been studied before. While an efficient offline algorithm for the classical paging problem is known, we neither have an efficient offline algorithm for min-max paging nor a proof of NP-hardness. In this paper, we focus on the min-max paging problem in the {\em online} setting and give both upper and lower bounds on its competitive ratio. 

\paragraph{Our results} We first propose an algorithm for the \textit{fractional paging problem} with objective function $f$, where pages can be held in the cache fractionally, subject to having a total volume of at most $k$ pages at all times. The objective function $f$ is an arbitrary function from an appropriately defined subclass of convex functions applied to the \textit{fault vector}. Here, the fault vector refers to the $n$-dimensional vector of the number of faults incurred on each page, where $n$ is the number of pages. We use the theory of convex programming and properties of $f$ to analyze our algorithm and establish the following bound.
\begin{theorem}[Stated formally as Theorem~\ref{thm:frac}]
For the fractional paging problem with objective function $f$, there exists a $(2q\log(k+1))^q$-competitive algorithm, provided $f$ grows no faster than a degree-$q$ polynomial.
\end{theorem}
In particular, when instantiating $f$ to be the $q$'th power of the $q$-norm, we get the following bound:
\begin{restatable}[Stated formally as Theorem~\ref{qpaging}]{theorem}{qpaging}
For the fractional paging problem with the objective of minimizing the $\ell_q$-norm of the fault-vector, there exists a $2q\log(k+1)$-competitive algorithm.
\end{restatable}
Note that the above theorem does not give a sensible result for the $\ell_\infty$-norm, which is the objective function we are interested in. However, using the fact that the $\ell_\infty$-norm of an $n$-dimensional vector is well-approximated by its $\ell_{\log(n)}$-norm, we get the following result.
\begin{theorem}[Stated formally as Theorem~\ref{thm_frac_ub}]
For the fractional paging problem with the objective of minimizing the $\ell_\infty$-norm of the fault-vector (a.k.a. fractional min-max paging), there exists an $O(\log(n)\log(k))$-competitive algorithm.
\end{theorem}
Next, we propose two approaches for rounding solutions of fractional min-max paging algorithms online and obtain the following two results. Note that the bound of the latter result is better than the former in the $k=\omega(\log n)$ regime, and it also rules out a lower bound linear in $k$ for randomized algorithms.
\begin{theorem}[Stated formally as Corollary~\ref{detround}]
  There exists an $O(k \log(k) \log(n))$-competitive {\em deterministic} algorithm for min-max paging.
\end{theorem}
\begin{restatable}[]{theorem}{randomizedfinal}
  There exists an $O(\log^{2}n \log k)$-competitive {\em randomized} integral algorithm for min-max paging.
  %There is an $O(\log(k) \log^2(n))$-competitive {\em randomized} algorithm for min-max paging.
\end{restatable}
We complement the above upper bounds by the following impossibility results.
\begin{theorem}[Stated formally as Theorem~\ref{thm:detlb}]
  Every deterministic algorithm for min-max paging is $\Omega(k \linebreak[2] \log(n)/ \log(k))$-competitive.
\end{theorem}
\begin{theorem}[Stated formally as Theorem~\ref{thm_lb}]
  Every algorithm for min-max paging is $\Omega(\log(n))$-competitive.
\end{theorem}
Note that we only have a $O(\log^2k)$ discrepancy between our deterministic bounds, i.e., the bounds are tight up to a polylogarithmic in $k$ factor. Moreover, our lower bounds show that min-max paging is fundamentally more difficult than classical paging and its several generalizations (see Section~\ref{sec:related-work}), which admit competitive ratios independent of $n$, the total number of pages.

%\subsection{Paging and MinMax Paging}
%\label{sec:paging-min-max-paging}

%  \ac{This should go to the concluding remarks section. For min-max paging, we give a rounding technique (see Section~\ref{sec:round}), to get a $Ck$-competitive algorithm using a $C$-competitive randomized algorithm.  This leads us to the following essence of our lower-bound result. }
%\begin{center}
%\begin{minipage}{0.9\textwidth}
%\begin{mdframed}[hidealllines=true, backgroundcolor=gray!15]
%\ac{  Competitive ratios of paging and min-max paging are separated by a factor of
%  $\log (n)/ \log(k)$ and by $\log (n)/ \log^2(k)$ in the randomized setting.}
%\end{mdframed}
%\end{minipage}
%\end{center}
We now present some intuition why algorithms for the classical paging problem and a simple algorithm for min-max paging fail to achieve anything better than a trivial competitive ratio for min-max paging. Algorithms for the classical paging problem are oblivious to the number of faults a single page has incurred while processing the sequence $\sigma$ up to a given point in time $t$. Consider the Least Recently Used (LRU) algorithm, which evicts the page whose last request was before the requests to other pages in the cache. Let $p_0 \in P = \{p_0, p_1, \dots, p_n\}$ and assume that $n = |P| - 1 = mk$ is a large multiple of $k$. The sequence $\sigma = (p_0, p_1,p_2, \dots, p_k, p_0, p_{k+1}, p_{k+2}, \dots, p_{2k}, p_0, p_{2k+1}, \dots, p_{mk}, p_0)$ will cause the LRU algorithm to fault $m + 1$ times on page $p_0$, while the optimal algorithm faults exactly once per page. We pair each request to $p_0$ with requests to a set of $k$ pages. After processing these $k$ requests, LRU will have ejected $p_0$, so the next request to $p_0$ will result in a page fault, yielding in a competitive ratio of $\Omega(n/k)$.

Another obvious strategy is to greedily keep the $k$ pages which have incurred the most faults thus far in the cache. In this case, there also exists a request sequence for which the strategy is no better than $\frac{n}{k}$-competitive. For simplicity's sake, let us assume that $k=2$. Then the request sequence is constructed as follows:
(1) Request $p_1, p_2, p_3$ in this order $N$ times, where $N$ is a parameter.
(2) Request $p_4, p_5$ until the algorithm includes \emph{both} of them into the cache.
(3) Request $p_4, p_5, p_6$ in this order $N$ times.
(4) Repeat steps 2 and 3 with pages $p_7$, $p_8$, and $p_9$ next, then with pages $p_{10}$, $p_{11}$, and $p_{12}$, and so on.

After step 3, the greedy algorithm will hold two pages of cost $(r+1)N$, where $r$ is the number of times we have repeated steps $2$ and $3$. In step 2, we request a set of new pages, and the greedy algorithm will fault on them until they reach cost $(r+1)N$. During step $3$, the algorithm will fault $N$ times on each page, making it so that it has cost $(r+2)N$ on the pages introduced in step $2$. Meanwhile, the cost of the optimal offline algorithm is no greater than $N$, obtained by immediately adding the pages of step 2 to the cache.
%We now try to gauge how some obvious attempts at solving min-max paging using ideas from paging fail. First, we discuss the marking algorithm. It marks and unmarks pages.  Initially, all pages are unmarked.  Whenever a request for page~$p$ arrives, if $p$ is in the cache and is unmarked, it gets marked. If $p$ is not in the cache, an unmarked page from the cache is evicted using some rule (or think arbitrarily).  If there is no unmarked page to evict, all the pages in the cache are unmarked, and the rule is applied. The new page is marked immediately upon being put in the cache. In the randomized marking algorithm, an unmarked page is chosen uniformly at random for eviction.  Now, we can design a request sequence where the marking algorithm will \emph{always} fault on every request to a fixed page, say $p_1$. E.g., suppose $k = 2$ and the rule we use is \emph{least recently used}, i.e. if there are multiple unmarked pages for possible eviction, we choose the one whose latest request was farthest in the past. Consider the request sequence $p_1, p_2, p_3, p_1, p_4, p_5, p_1, p_6, p_7,\ldots, p_1, p_{n-1}, p_n$. It can be seen that the number of page faults on $p_1$ is about $n/2$ (i.e., $n/k$), whereas on the other pages it is $1$.  This is much worse than when we always keep $p_1$ in the cache, incurring a cost of only~$1$. This example suggests another greedy approach. Evict the page in the cache, which has incurred the smallest number of page faults. Unfortunately, this strategy also does not work. Consider the following request sequence; again, $k = 2$.
% \begin{enumerate}
%   \item Request $p_1, p_2, p_3$ in this order $N$ times, where $N$ is a parameter.
%   \item Request $p_4, p_5$ until the algorithm puts \emph{both} of them in the cache.
%   \item Request $p_4, p_5, p_6$ in this order $N$ times.
%   \item Repeat steps 2 and 3 with pages $p_7$, $p_8$, and $p_9$ next, then with pages $p_{10}$, $p_{11}$, and $p_{12}$, and so on.
% \end{enumerate}
% For every request to the two new pages introduced in step~2, the greedy faults, whereas a good strategy is to bring them into the cache immediately. Thus, the cost of the greedy increases by $cN$ for some constant $c$ in each of the $n/3$ (i.e., $n/(k+1)$) iterations, whereas the cost of an optimal offline algorithm is about $N$.

% Ashish: Contrast with paging: why don't usual techniques work? (Optional:
% mention our techniques. Personally, I don't like attempts to mention
% techniques in the intro; they turn out to be too vague for me to make
% sense. But apparently, some readers like that.)

\paragraph{Our techniques}
Our lower bound of $\Omega(k \log(n)/ \log(k))$ is established by generalizing the above construction, using the following approach: The adversary fixes a sequence of requests over a set of $n$ pages, which can be served while keeping the number of faults on any page small. The core idea is to successively reduce the set of pages that we request in the future in such a way that the algorithm \emph{cannot predict which pages will stop being requested.} A clairvoyant adversary processes the sequence so that she initially incurs a small number of faults on pages that will be requested many times in the future. This causes the adversary to have roughly uniform cost over all pages, while the algorithm has one page on which it has faulted many times.

To design an online algorithm 
%or the online min-max paging problem, 
one could try to use  standard techniques to transform a max-based objective function into a linear program and solve the corresponding linear program online. However, this  does not work as all known online algorithms for linear programs only work with {\em exclusively packing or exclusively covering constraints} and can not handle a mix of constraints, except for~\cite{azar2013online}, which cannot handle {\em box constraints,} i.e., an upper bound on the variables as required for paging.

Thus, to solve the online min-max paging problem, we solve a more general problem: We give a $O((q\log k)^q)$-competitive  algorithm for a \emph{fractional  paging problem, which minimizes a convex, differentiable function with $q$-bounded growth} and \emph{an upper bound constraint (i.e., a box constraint) on each variable.} A function with $q$-bounded growth behaves like a polynomial function of degree $q$.
To the best of our knowledge, this problem has not been studied before, and no non-trivial online algorithm is known.

As our cost function is not linear, the combinatorial technique of potential functions used for server problems with linear cost functions breaks down. Informally, a potential function captures the advantage accumulated by the adversary at any time, which she can use to make the algorithm ``pay'' more than herself in the future. The potential function is a function on the \textit{state space} of the problem, where the state of the algorithm, at any time, fully determines its future behavior. The state space is usually a small set when the objective is linear. On the contrary, in the case of min-max paging, a state must capture the vector of faults accumulated on each page and its current cache, and there can be multiple fault vectors for the same current cache, which makes the state space blow up with every request, thus, making the use of potential functions challenging, messy, and inelegant.

Instead, we build on the work of Azar~et~al.~\cite{azarOnlineAlgorithms2016}, which minimizes a convex cost function with linear constraints of \emph{row sparsity} $\rho$. Their approach requires the variables $x_{p,j}$ to be unbounded, and for $q$-bounded growth functions, it gives an $O((q\log\rho)^q)$-competitive algorithm. 
% In our setting, $\rho$ equals $n$, i.e., a straightforward application of their algorithm would give a $O((q\log n)^q)$-competitive algorithm without box constraints. 


We also draw on ideas from Bansal et al.~\cite{bansalbn_12}, which  studied the weighted paging problem with linear cost functions.
They first compute a fractional solution using a primal-dual approach and then show how to round it.
As they have a linear cost function, they can show that the rate of increase of the primal, i.e., the fractional algorithm's cost, is proportional to the rate of increase of the dual.
In our setting, the cost function is not linear, and we have to use the theory of duality of convex programs and conjugate duals. To do so, we extend their analysis to the convex program setting, which requires solving various technical hurdles. This results in a $(2q \log (k+1))^q$-competitive algorithm for fractional paging with any  convex, differentiable function with $q$-bounded growth and box constraints.
Furthermore, for norm-objective functions, more specifically for $q$-norms, we achieve a  competitive ratio of $2q \log k$.
Since the cost function of min-max paging is the $\ell_\infty$-norm of the vector of page-wise costs, we approximate it by $\ell_{\log n}$-norm, resulting in a $2e \log n \log(k+1)$-competitive algorithm
for fractional min-max paging.

We round our solution deterministically using for every page $p$ a threshold  for $x_p$of $1-1/k$, resulting in the upper bound of $O(k \log n \log k)$.
It might be tempting to apply the randomized rounding algorithm of~\cite{bansalbn_12} directly, but it does not apply as it crucially uses the fact that the cost of the algorithm is the sum of the fractional values of all pages.
Instead, we adapt the scheme of~\cite{bansal2021efficient} from the weighted paging setting to the  min-max setting. Specifically, this requires to ``charge'' the cost of each rounding step to each individual page, as opposed to the sum of the changes in the fractional solution over all pages. This charging to individual pages has not been done before in online paging and might be interesting in other settings.

%The rounding scheme consists of two steps and this requires a different analysis of the cost of one of these steps.



%\paragraph{Organization of the paper.}
In Section 2, we give all definitions.  In Section 3, we show our lower bounds,
%for min-max paging in both the deterministic and randomized settings. 
in Section 4, we present and analyze our algorithm for paging with convex objective functions.
%and use it to derive an upper bound for fractional min-max paging. 
In Section 5 we round the fractional algorithm to obtain an $O(k \log(n) \log(k))$-competitive deterministic and $O(\log^2 (n) \log(k))$-competitive randomized algorithms for (integral) min-max paging. All omitted proofs  are given in the appendix.

%\sag{Someone: organization of the paper once everything is finalized.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/lb.tex <==
\section{Lower Bounds}

\label{sec:lb}
We show a deterministic lower bound of $\Omega(k (\log n)/\log k)$ and a randomized lower bound of $\Omega(\log n)$ (for $k = 2$) on the competitive ratio for min-max paging.  Our lower bounds are based on a simple construction that is cleanly demonstrated with $k = 2$ and can be generalized for $k \ge 2$.
%We only discuss the instructive $k = 2$ cases here. 
The interested reader will find complete proof for the deterministic lower bound in the appendix in Section~\ref{app:lb}.

\begin{restatable}{@theorem}{detlb}
\label{thm:detlb}
Any deterministic algorithm for min-max paging with cache size $k$ is at least $\frac{k-1}{2} \log_{k+1} n$-competitive, where $n$ is the number of pages.
%The deterministic competitive ratio of min-max paging is $\Omega(k (\log n) / \log k)$, where $n$ is the number of pages.
\end{restatable}

\input{randlb.tex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/prelim.tex <==
\section{Preliminaries}

%\subsection{Competitive Analysis}

The problems in this paper are studied in the online setting, where an adversary fixes a request sequence $\sigma$ ahead of time, and the requests in this sequence are presented to an algorithm one by one. When the algorithm receives a new request from the sequence, it can only use its knowledge of the requests seen thus far to make a decision. In particular, the algorithm does not have any knowledge of future requests.

In this setting, we use \emph{competitive analysis} \cite{SleatorT85} to measure the quality of an algorithm. % TODO cite sleator tarjan [27] in buchbinder/bansal/naor weighted paging
In competitive analysis, we study the \emph{competitive ratio} of an online algorithm, which compares the worst-case ratio between the cost of the algorithm and the cost of an optimum offline solution over all possible $\sigma$.

More formally, for a deterministic algorithm $\ALG$, the competitive ratio of $\ALG$ is the smallest $c \in \mathbb{R}$, such that for all instances $\sigma$ of an online minimization problem, we have
\[
  \ALG(\sigma) \le c \cdot \OPT(\sigma) + d,
\]
where $\ALG(\sigma)$ is the cost of the algorithm, $\OPT(\sigma)$ is the cost of the optimum offline solution, and $d$ is some constant independent of $\sigma$. We will call an algorithm fulfilling the above definition a $c$-competitive algorithm. If $\ALG$ is a randomized algorithm, then the competitive ratio is defined as the smallest $c \in \mathbb{R}$ such that
\[
  \mathbb{E}[\ALG(\sigma)] \le c \cdot \OPT(\sigma) + d.
\]
%Note that we do not require this inequality to hold with high probability.

% 1. Definition of competitive ratio, make it specific to the paging problem?

%\subsection{Problem Definition}

We study a variant of the paging problem called \emph{min-max paging}. In any paging problem the request sequence $\sigma$ is made up of requests to a set of pages $P = \{p_{1}, p_{2}, \dots, p_{n}\}$ of size $n$. We will assume that $\sigma$ is of finite length, denoted by $T$. The algorithm is given a cache $C$ of size $k$, which always is a subset of $P$ and is empty when the algorithm begins processing $\sigma$.

When page $p$ is requested during round $t$, we must add $p$ to the cache $C$ if it is not already contained in $C$. If adding the page causes $C$ to be of size $k+1$, we must evict a page other than $p$ from the cache before we are allowed to process the next request. The situation where a request to page $p$ arrives while $p$ is not in $C$ is called a \emph{page fault}.

% 2. Formal defininition of problem with infinity norm
Whenever a page fault occurs, we incur some cost. The objective of the classical paging problem is to minimize the total number of page faults. In the case of min-max paging, the objective is to minimize the maximum number of page faults occurring for any page. More precisely, if we let $x_{p,j}$ be a zero-one variable, which denotes that a page fault occurs upon the $j$-th request to page $p$, then we seek to minimize
\[
  \max_{{p \in P}} \sum_{j} x_{p,j},
\]
where the summation is over all requests to $p$. We can think of this as minimizing the $\ell_{\infty}$-norm of the vector
$\vec{c}(\sigma) = (\sum_{j} x_{p_{1},j} , \dots, \sum_{j} x_{p_{n},j} )^\top$,
%\[
%  \vec{c}(\sigma) = \begin{bmatrix} \sum_{j} x_{p_{1},j} \\ \vdots \\ \sum_{j} x_{p_{n},j} \end{bmatrix},
%\]
whereas the classical paging problem is equivalent to minimizing the $\ell_{1}$-norm of $\vec{c}(\sigma)$.

% 3. More generally -> f-paging (refer to section 4 for the detailed properties of f)

In Section 4 we solve a fractional version of the paging problem for convex objective functions $f(x)$, where $x$ is the vector consisting of the variables $x_{p,j}$, under the assumption that $f(x)$ is well behaved. Of particular interest is the case where $f(x) = \|\vec{c}(\sigma)\|_{q}$, i.e. the $\ell_{q}$-norm. We refer to this case as \emph{$q$-paging}. For details refer to Section 4. % TODO make this a hyperlink to the definition of the function

% 1. Mention eviction cost and fetching cost models and their equivalence in our problem
\begin{Remark}
  % equivalence of eviction cost and fetching cost model
  Paging problems are studied in the eviction cost model, where fetching a page incurs no cost, and the algorithm pays for evicting a page, and in the fetching cost model, where evicting a page comes without an associated cost, and the algorithm pays for fetching a page. For min-max paging, the cost of these models differs by at most $1$. 
  %The pages where this difference occurs are those which remain in the cache at time $T$ and will not be evicted.
  Said difference occurs on the set of pages contained in the cache at time $T$ that the algorithm does not have to evict anymore.

  Because of this equivalence, we use both models interchangeably in this paper. The lower bounds of Section 3 use the fetching cost model, and the upper bounds of Section 4 use the eviction cost model, as the choice of the respective model simplifies the proofs.
\end{Remark}







% In the paging problem and its variants, we are given a set $P = \{p_{1}, p_{2}, \dots, p_{n}\}$ of pages and
% a cache $C$ of size $k$, which will always hold a subset of the pages.

% As paging is an online problem, we view it as a two-player game between an adversary and the
% algorithm. The goal of the adversary is to



% An algorithm for paging has a cache $C$ of size $k$, which, at any point in time must be a
% subset of $P$ of size at most $k$. Upon receiving a request to a page $p$, the
% algorithm must add the requested page $p$ to its cache, if it is not already present in $C$,
% before the next request from $\sigma$ is revealed. If adding the page $p$ to $C$ causes the cache to contain more than
% $k$ pages, a page other than $p$ must be evicted from the cache in order to make room
% for $p$.

% When a page is not in the cache when it is requested, we say a page fault occurs and
% we incur some cost.










% In the \emph{weighted paging} problem, we are given a set of pages
% $P = \{p_1, \dots, p_n\}$ and for each page $p \in P$, its weight $w_p$.  There
% is a cache of size $k$.  We are also given a request
% sequence $\sigma \in P^T$ of length $T$; we need to process $\sigma$ while
% maintaining the following invariants:
% \begin{enumerate}
%   \item After processing the $t$th element $p_t$ of the sequence, it must be in
%   the cache.
%   \item After processing $p_t$, the cache can contain at most $k$ pages.
% \end{enumerate}
% Hence, if page $p$ is not in the cache when it is requested, we need to
% \emph{evict} some other page to make room for $p$; we call this a \emph{page
%   fault}, and we incur a cost of $w_p$.  (Otherwise, we incur no cost.)
% Then, the goal is to minimize the total cost incurred while maintaining
% the invariants stated above.
% % The strategy by which an algorithm evicts pages
% % fully defines its behavior and competitiveness.

% We call the processing of $t$th element or $t$th \emph{request} of $\sigma$ as
% $t$th \emph{round}.  For $t \in [T]$, where $[T] := \{1, 2, \ldots, T\}$, let
% $c_p(t)$ denote the number of page faults after a request to page $p$ after $t$
% rounds.  The \emph{cost vector} $\mathbf{c}(t)$ at round $t$, is defined as:
% $\mathbf{c}_p(t) = w_p c_p(t)$.

% The weighted paging problem then asks to minimize the $\ell_1$-norm of
% $\mathbf{c}(T)$.  In this paper, we generalize this to minimizing
% $\|\mathbf{c}\|_q$ for $q \in (1, \infty]$. %\sag{Need to use a symbol other than
%   %$p$.}  Max: Changed symbol to q, as is used later in the paper.
%   In particular, we call the case of $q = \infty$ as the \emph{min-max
%   paging} problem, as it corresponds to minimizing
% $\max_{i \in [n]} \mathbf{c}_i(T)$, which is closely related to the popular
% notion of max-min fairness from network algorithms.

% \mx{Should we add this as a definition in the preliminaries, it does not fit with the definition of the convex primal any more? It fits with the cost vector motivation.}In the case of $f(x) = \left( \sum_{p \in P} \left( \sum_{j=1}^{r(p,T)} x_{p,j}\right)^q \right)^{\frac1q}$,
% we call
% the resulting problem \emph{$q$-paging}.

% \sag{TODO (Ashish): Need to add definition of online, offline algos, competitive ratio.}

% % An example of an application where this kind of fairness might be desirable is
% % deciding which TCP connections to keep alive on a server, as guaranteeing
% % clients that they do not have to re-establish connections too many times
% % provides a Quality of Service guarantee.

% \subsection{A Linear Program (LP) for Paging}

% We borrow the LP and notation from Bansal et al.~\cite{bansalbn_12}.  For
% $p \in P$ and $j \in \N$, let $t(p, j)$ denote the request number of $j$th
% request to $p$.  For $t \in [T]$, let $B(t)$ the set of pages seen until request
% number $t$, i.e., $B(t) = \{p \in P : t(p,1) \le t\}$.  For $p \in P$ and
% $t \in [T]$, let $r(p,t)$ denote the number of requests to $p$ until (inclusive)
% $t$.  We consider the following integer linear program (ILP) for weighted
% paging, where the variable $x_{p,j}$ indicates that $p$ has been removed from
% the cache between its $j$th and $(j{+}1)$th requests.

% \begin{equation*}
%   \begin{array}{lll}
%     \text{minimize } & \sum_{p,j} w_p x_{p,j} &  \\
%     \text{subject to } & \sum_{p \in B(t) \setminus \{p_t\}} x_{p, r(p,t)} \ge |B(t)| - k & \forall t \in [T] \\
%                      & x_{p,j} \in \{0, 1\} & \forall p \in [n], j \in [r(p,T)]. \\
%   \end{array}
% \end{equation*}
% Hence, if $x_{p,j} = 1$, we incur a cost of $w_p$ to move the page $p$ back into
% the cache on the $(j{+}1)$th request.  The first constraint tells us that during
% any round, we must evict at least $|B(t)| - k$ pages from the cache to keep the
% number of pages in cache $\le k$.

% In the LP relaxation of the above ILP, the constraints $ x_{p,j} \in \{0, 1\}$
% are replaced by $0\le x_{p,j} \le 1$.  A non-integral solution to the LP gives
% us a \emph{fractional} algorithm for paging, where a fraction of a page can be
% in the cache, and the remaining fraction is outside the cache.  The requirement
% that a page be completely in the cache after a request to it is satisfied by
% even a non-integral solution to the LP.

% \sag{TODO: The following should go in the introduction.}
% \paragraph{Note} Fair paging can be expressed as an ILP using a standard trick:
% add one constraint for each page with variable $L$ denoting an upper bound on
% its ``cost,'' then minimizing $L$.

% %\sag{Max, Can you please elaborate what the exact issue is?}
% However, the resulting
% structure of the constraint matrix, makes it challenging to apply existing frameworks for online linear programming such as \cite{buchbinder2009online}, as these frameworks only apply to strict covering or packing linear programs, i.e. those in which the constraint matrix has either all positive or all negative entries.



% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:


==> MinMax (Fair) Paging/randlb.tex <==
%\subsection{Randomized Lower Bound}
%\paragraph{Randomized Lower Bound}
\begin{theorem}\label{thm_lb}
  The randomized competitive ratio of min-max paging is $\Omega(\log n)$, where $n$ is the number of pages when the cache size is $k=2$.
\end{theorem}

By Yao's principle, it suffices to exhibit a probability distribution on input instances, forcing every deterministic online algorithm to perform a factor $\Omega(\log n)$ worse in expectation than the optimum cost. Let $n=3^m$ for some large integer $m$. Our adversarial strategy takes a parameter $N\gg n$ and is defined as follows.
\begin{algorithm}
  \caption{An adversarial strategy for min-max paging}\label{adversary}
  \begin{algorithmic}[1]
    \State Let $L_m=\{p^m_0,\ldots,p^m_{n-1}\}$ be a set of $n=3^m$ pages.
    \For{$\ell$ $=$ $m$ to $1$} \State $L_{\ell-1}\gets\emptyset$.  \For{$i$ $=$
      $0$ to $3^{\ell-1}-1$} \State Give $N$ requests to each of
    $p^{\ell}_{3i},p^{\ell}_{3i+1},p^{\ell}_{3i+2}$ in a round-robin manner.
    \State $p^{\ell-1}_i$ $\gets$ a uniformly random page from
    $\{p^{\ell}_{3i},p^{\ell}_{3i+1},p^{\ell}_{3i+2}\}$.  \State Add
    $p^{\ell-1}_i$ to $L_{\ell-1}$.  \EndFor \EndFor
  \end{algorithmic}
\end{algorithm}

We call each iteration of the outer for-loop a \textit{layer} and each of the inner for-loop a \textit{phase}. We number the layers $m,m-1,\ldots,1$.

% \begin{obs}
%   In each phase of layer $\ell$, three pages are removed from $L_{\ell}$ and
%   one of them is added to $L_{\ell-1}$. Therefore, $|L_{\ell}|=3|L_{\ell-1}|$,
%   and thus, $|L_{\ell}|=3^{\ell}$.
% \end{obs}

\begin{lemma}\label{lem_lb_adv}
  The adversary can serve all requests while faulting at most $m+N$ times on every page with probability one.
\end{lemma}
\begin{proof}
  Consider an arbitrary phase of an arbitrary layer $\ell$. Let $q$ be the page added to $L_{\ell-1}$ at the end of the phase, and let $q_1,q_2$ be the other two pages requested in the phase. On the first request to $q$, the adversary will add $q$ to its cache and keep it there until the end of the phase. It uses the remaining cache slot to serve all requests to $q_1$ and $q_2$. Thus, the adversary faults only once on $q$ and $N$ times on $q_1$ and $q_2$ each.

  Consider an arbitrary page $p$. In all phases where $p$ is requested except the last one, the adversary faults only once on $p$ ($p$ is the page $q$ in the above argument). In the last phase, the adversary faults $N$ times on $p$. Every layer contains at most one phase in which $p$ is requested. Since the number of layers is $m$, the algorithm faults at most $m+N$ times on $p$.
\end{proof}

To analyze the algorithm's performance, let the random variable $X^{\ell}_i$ be the number of the algorithm's faults on the randomly chosen page $p^{\ell}_i$ at the beginning of layer $\ell$.

\begin{lemma}\label{lem_lb_alg}
  For every layer $\ell$ and every $i\in\{0,\ldots,3^{\ell}-1\}$ we have $\mathbb{E}[X^{\ell}_i]\geq(m-\ell)\cdot N/2$.
\end{lemma}

\begin{proof}
  We prove the claim by reverse induction on $\ell$. Recall the numbering of phases and observe that $X^m_i=0$ for all $i\in\{0,\ldots,n-1\}$. Thus, the claim is true for $\ell=m$. Assuming as induction hypothesis that for every $i\in\{0,\ldots,3^{\ell}-1\}$ we have $\mathbb{E}[X^{\ell}_i]\geq(m-\ell)\cdot N/2$, we prove that for every $j\in\{0,\ldots,3^{\ell-1}-1\}$ we have $\mathbb{E}[X^{\ell-1}_j]\geq(m-\ell+1)\cdot N/2$.

  In any phase, since the cache size is $2$ and three pages are requested in a round-robin manner $N$ times each, the total number of faults is at least $3N/2$. This is evident if we consider the behavior of the optimal algorithm for (usual) paging that always evicts the page needed farthest in the future. Consider the $j$'th phase of layer $\ell$, and recall that $p^{\ell-1}_j$ is defined at the end of this phase. The total number of faults in this phase is at least $3N/2$, and these faults are distributed over the three pages, $p^{\ell}_{3j},p^{\ell}_{3j+1},p^{\ell}_{3j+2}$. Since $p^{\ell-1}_j$ is uniformly random among these three pages, the expected number of faults on $p^{\ell-1}_j$ during layer $\ell$ is at least $N/2$. Again, since $p^{\ell-1}_j$ is uniformly random among $\{p^{\ell}_{3j},p^{\ell}_{3j+1},p^{\ell}_{3j+2}\}$, by linearity of expectation we have,
  \[\mathbb{E}[X^{\ell-1}_j]\geq\frac{\mathbb{E}[X^{\ell}_{3j}]+\mathbb{E}[X^{\ell}_{3j+1}]+\mathbb{E}[X^{\ell}_{3j+2}]}{3}+\frac{N}{2}\text{.}\]
  By the induction hypothesis, each of $\mathbb{E}[X^{\ell}_{3j}]$, $\mathbb{E}[X^{\ell}_{3j+1}]$, $\mathbb{E}[X^{\ell}_{3j+2}]$ is at least $(m-\ell)\cdot N/2$. Thus, $\mathbb{E}[X^{\ell-1}_j]\geq(m-\ell+1)\cdot N/2$, as required.
\end{proof}

Having proven Lemma~\ref{lem_lb_adv} and Lemma~\ref{lem_lb_alg}, we are ready to prove the claimed lower bound.

\begin{proof}[Proof of Theorem~\ref{thm_lb}]
  By Lemma~\ref{lem_lb_adv}, the cost of the adversary's solution to the random instance generated by the adversarial strategy is $m+N$ with probability one. Note that at the end of the adversarial strategy, we are left with the singleton set $L_0$ containing the page $p^0_0$. The number of faults of the algorithm on page $p^0_0$ is a lower bound on the algorithm's cost with probability one. Thus, the algorithm's expected cost is at least the expectation of the number of algorithm's faults on $p^0_0$. By Lemma~\ref{lem_lb_alg}, this quantity is $\mathbb{E}[X^0_0]\geq mN/2$. Thus, the ratio of the algorithm's expected cost to the adversary's cost is at least $mN/(2\cdot(m+N))$, which approaches $m/2=(\log_3n)/2$ as $N\rightarrow\infty$. Thus, the competitive ratio of any randomized algorithm for min-max paging is at least $(\log_3n)/2=\Omega(\log n)$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> MinMax (Fair) Paging/related-work.tex <==
\section{Further related work}\label{sec:related-work}

Sleator and Tarjan~\cite{SleatorT85} defined the framework of online algorithms and competitive analysis, and paging is one of the earliest problems studied in the online setting. Several deterministic algorithms, such as ``Least Recently Used'' (LRU) and ``First In First Out'' (FIFO), among others, are known to achieve the optimal deterministic competitive ratio of $k$~\cite{SleatorT85}, where $k$ is the maximum number of pages that can be inside the cache at any point in time. The randomized competitive ratio is known to be $H_k$, where the upper bound is due to Achlioptas et al.~\cite{AchlioptasCN_TCS00} and the lower bound is due to Fiat et al.~\cite{FiatKLMSY_JAlg91}.

Several practical generalizations of the paging problem have been studied and they are known to have a deterministic competitive ratio of $k$~\cite{ChrobakKPV90,Young98} and randomized competitive ratio $\Theta(\log k)$~\cite{bansalbn_12,BansalBN12_sicomp}. These include weighted paging -- where pages have arbitrary loading costs, the \textit{bit model} -- where pages have arbitrary sizes and loading cost proportional to size, the \textit{fault model} -- where pages have arbitrary sizes but unit loading cost, and generalized paging -- where pages have arbitrary loading costs as well as sizes. Interestingly, all these results are robust in the sense that they all extend to the resource-augmentation setting, where the adversary has fewer servers than the algorithm. It is noteworthy that the line of work in search of a randomized algorithm for these paging variants by Bansal, Buchbinder, and Naor led to the development of the online primal-dual framework for designing fractional algorithms for online problems, whose solutions can often be rounded to an integral solution online.

A simple-looking but intriguing generalization of paging is the $k$-server problem defined by Manasse, McGeogh, and Sleator~\cite{ManasseMS88}, which concerns moving $k$ mobile servers on a metric space to serve requests while minimizing total movement. (The paging problem is the $k$-server problem on the uniform metric over the set of pages.) While Manasse et al.~\cite{ManasseMS88} proved a lower bound of $k$ on the deterministic competitive ratio for every metric space with more than $k$ points, the existence of a $k$-competitive algorithm is still unknown, and this is popularly called the $k$-server conjecture. The best-known $k$-server algorithm that works for all metrics called the \textit{Work Function Algorithm} by Koutsoupias and Papadimitriou~\cite{KoutsoupiasP95}, achieves a competitive ratio of $2k-1$. For randomized algorithms, surprisingly, neither a better upper bound than the deterministic $2k-1$ nor a better lower bound of $\Omega(\log k)$ arising from paging is known. Koutsoupias~\cite{Koutsoupias09} presents a more comprehensive discussion on the $k$-server problem.


==> MinMax (Fair) Paging/rounding.tex <==
\section{Rounding Fractional Solutions Online}\label{sec:round}

\subsection{\texorpdfstring{An $O(k \log(n) \log(k))$-competitive Deterministic Algorithm}{An O(k log(n) log(k))-competitive Deterministic Algorithm}}

This section shows how to round a fractional solution for min-max paging to an integral solution online. The rounding procedure is deterministic and, when coupled with a fractional min-max paging algorithm, gives a deterministic min-max paging algorithm.

\begin{theorem}\label{thm_rounding}
If there exists an $\alpha$-competitive algorithm for fractional min-max paging with cache size $k$, then there exists a $(\alpha k)$-competitive deterministic algorithm for min-max paging with cache size $k$.
\end{theorem}

\begin{proof}
Without loss of generality, we assume that the fractional min-max paging algorithm is lazy. That is, it loads a page only when the page is requested. Indeed, an arbitrary solution can be converted into a lazy solution online without increasing the cost by delaying page loads as much as possible.

The deterministic integral algorithm maintains the following invariant: it always has a page $p$ in its cache whenever the fractional algorithm has more than a $1-1/k$ fraction of $p$ in its cache. We observe that the fractional algorithm must always fully have at least one page in its cache: the most recently requested page. Therefore, at any time, the number of pages $p$ such that the fractional algorithm contains more than a $1-1/k$ fraction of $p$ is less than $1+(k-1)/(1-1/k)=k+1$, and therefore, this number is at most $k$.

Consider an arbitrary request to some page $p$. If the integral algorithm already has $p$ in its cache, it ignores the request, whereas the fractional algorithm possibly serves the request by evicting some pages fractionally. On the other hand, suppose the integral algorithm does not already have $p$ in its cache, then this implies that the fractional algorithm has at most a $1-1/k$ fraction of $p$ in its cache. After the fractional algorithm brings $p$ into its cache, the integral algorithm must have a page $q$ in its cache such that the fractional algorithm has at most a $1-1/k$ fraction of $q$ in its cache. (Otherwise, the fractional algorithm has more than a $1-1/k$ fraction of $k+1$ pages in its cache, namely, the $k$ pages in the integral algorithm's cache and the page $p$, thus contradicting the observation from the last paragraph.) The integral algorithm replaces one such page $q$ by $p$ to serve the request and thus, maintains the invariant. In this process, the integral and the fractional algorithms incur $1$ and at least $1/k$ faults, respectively, on page $p$.

Thus, at the end of the request sequence, for every page $p$, the number of faults of the integral algorithm on $p$ is at most $k$ times the number of faults of the fractional algorithm on $p$. Thus, the cost of the integral algorithm is at most $k$ times the cost of the fractional algorithm. Since the latter is at most $\alpha$ times the cost of the optimum, the cost of the integral algorithm is at most $\alpha k$ times the cost of the optimum solution.
\end{proof}

\begin{corollary}\label{detround}
There exists a $2ek\log(n)\log(k+1)$-competitive deterministic algorithm for min-max paging.
\end{corollary}

\begin{proof}
Follows from Theorem~\ref{thm_frac_ub} and Theorem~\ref{thm_rounding}.
\end{proof}

It is noteworthy that the trick in the proof of Theorem~\ref{thm_rounding} can also be used for the derandomization of randomized algorithms. Specifically, suppose an $\alpha$-competitive randomized algorithm exists for min-max paging. Then there also exists a fractional one with the same competitive ratio. Thus, by Theorem~\ref{thm_rounding}, there exists a $\alpha k$-competitive deterministic algorithm for min-max paging.


\subsection{\texorpdfstring{An $O(\log^{2}(n) \log(k))$-competitive Randomized Algorithm.}{An O(log2(n) log(k))-competitive Randomized Algorithm.}}

Using a more sophisticated rounding approach, we obtain a randomized algorithm whose competitive ratio no longer depends linearly on $k$, in exchange for an additional $\log(n)$ factor. This result rules out a lower bound of $\Omega(k)$. This algorithm is of interest in the regime where $\log(n) \le k$, which is often the case in applications.

%\ac{Max, since $n\geq k$, this is simply $O(\log^2n\cdot\log k)$. Also, mention right away which regime this algorithm is interesting in.}

We can obtain a randomized algorithm for min-max paging by using the rounding scheme for weighted paging of Bansal et al.~\cite{bansal2021efficient}.
%The rounding scheme is presented in
%Just like us, they have a variable $x_p(t)$ that indicates for each page how much of page $p$ we have ejected from the cache at time $t$.
The simplified rounding scheme is presented in Algorithm~\ref{randround}. 
Each online rounding step only depends on the previous, and current fractional cache states $x(t-1)$ and $x(t)$
as well as the previous integral cache state and  on a parameter $\beta$, which indicates how aggressively we eject pages from the cache.
\emph{The rounding scheme works for any caching scheme that fulfills the condition that (1) at any time $t$, for any page $p \ne p_r$, $x_p(t) - x_p(t-1) \ge 0$ and (2) the total fraction of pages evicted upon any request is at most 1.
} Algorithm~\ref{fractional} indeed has these properties, so we can use the rounding scheme as long as we can relate the rounding costs to our target function, even though we solve a different paging problem than they do.

Let $x$ be a fractional solution produced by Algorithm~\ref{fractional}. After processing round $t$, the algorithm will produce a fractional value $x_p(t)$ for each page, indicating the fraction of page $p$ in the cache in this round. In other words, the process of solving the fractional problem online produces, whenever Algorithm~\ref{fractional} finishes processing a round at time $\tau(t)$, the vector
\[
  x(t) = \begin{bmatrix} x_{p_{1},r(p,t)}(\tau(t)) \\ \vdots \\ x_{p_{n},r(p,t)}(\tau(t)) \end{bmatrix}.
\]
%We note that for two vectors $x(t)$ and $x(t+1)$, only one coordinate can decrease between rounds $t$ and $t+1$, namely the coordinate associated with $p_t$. All other coordinates can not decrease between rounds.

We let $y_p(t) = \min\{\beta \cdot x_p(t), 1\}$ be the solution in which every coordinate is scaled up by a factor of
$\beta$. The factor $\beta$ governs how much more aggressively pages are evicted from the cache.

Algorithm~\ref{randround} may evict pages and incur costs in two separate places. The first type we need to account for is the cost incurred via the random evictions of pages in the for-loop in lines 4-5 of the algorithm. The second type is the cost incurred by fixing the cache size in lines 6-7 if no page was evicted in the for-loop. We will bound these costs separately and combine them in our upper bound.

\begin{algorithm}
  \caption{The randomized rounding scheme of~\cite{bansal2021efficient} adapted to our problem.}\label{randround}
  \begin{algorithmic}[1]
    \Procedure{Round}{$x(t), x(t-1), C(t - 1)$}
    \If{$p_{t} \notin C(t - 1)$}\Comment{Add the page $p_{t}$ to the cache, if it is not already in it.}
    \State $C(t - 1) \gets C(t-1) \cup \{p_{t}\}$
    \EndIf

    \For{$p \in C(t-1) \setminus \{p_{t}\}$}
    \State Evict $p$ from $C(t-1)$ independently with probability $\frac{y_{p}(t) - y_{p}(t-1)}{1 - y_p(t-1)}$
    \EndFor

    \If{$|C(t-1)| > k$}%\Comment{If nothing was ejected in the previous step, we may need to eject a single page from $C(t-1)$ to guarantee $|C(t-1)| \le k$.}
    \State Evict an arbitrary page $p \neq p_{t}$ from $C(t-1)$
    \EndIf

    \State $C(t) \gets C(t-1)$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

For the first type, it is easy to see that the cost incurred for evicting a page in lines 4-5 depends only on the sequence of fractional values $y_{p}(1), y_{p}(2), \dots, y_{p}(T)$ that this page takes on and it is independent of the values $y_{p'}(t)$ for all $t$ and $p'\neq p$. In particular, the probability $y_{p,j}$ that a page is evicted
in lines 4-5, between its $j$-th and $j+1$-st request is
\begin{align*}
    \sum_{t=t(p,j)+1}^{t(p,j+1)-1} \Pr[\text{page $p$ is evicted in round $t$}] &=
    \sum_{t=t(p,j)+1}^{t(p,j+1)-1} \frac{y_p(t) - y_p(t-1)}{1 - y_p(t-1)} \Pr[\text{page $p$ is not evicted until round $t$}]\\
    & = \sum_{t=t(p,j)+1}^{t(p,j+1)-1} \frac{y_p(t) - y_p(t-1)}{1 - y_p(t-1)} \prod_{t'=t(p,j)+1}^{t-1} 1 - \frac{y_p(t') - y_p(t'-1)}{1 - y_p(t'-1)}\\
    & = \sum_{t=t(p,j)+1}^{t(p,j+1)-1} \frac{y_p(t) - y_p(t-1)}{1 - y_p(t-1)} \prod_{t'=t(p,j)+1}^{t-1} \frac{1 - y_p(t')}{1 - y_p(t'-1)} \\
    & = \sum_{t=t(p,j)+1}^{t(p,j+1)-1} \frac{y_p(t) - y_p(t-1)}{1-y_p(t(p,j))} = \frac{y_p(t(p,j+1)-1)}{1-y_p(t(p,j))} = y_{p}(t(p,j+1)-1).
\end{align*}
The second equation holds because of the independence of the probability of eviction in different rounds; the fourth holds because it is a telescoping product, and the last equation holds as $y_p(t(p,j)) = 0$.
Let $Y_{p,j}$ be a Bernoulli random variable that is $1$ with probability $y_p(t(p,j+1)-1)$ and let $Y_{p} = \sum_{j} Y_{p,j}$ be the sum of all $Y_{p,j}$ for fixed $p$. We let these variables track the expected cost of evictions for each page. By linearity of expectation, we immediately see that
\[
\mathbb{E}[Y_p] = \mathbb{E} \left[ \sum_{j=1}^{r(p,T)} Y_{p,j} \right] = \sum_{j=1}^{r(p,T)} \Pr[\text{$p$ is evicted between request $j$ and $j+1$}] = \sum_{j=1}^{r(p,T)} y_{p,j} \le \beta  \sum_{j=1}^{r(p,T)} x_{p,j}.
\]
It follows that
\[
\max_p \mathbb{E}[Y_p] \le \beta \max_p \sum_{j=1}^{r(p,T)} x_{p,j},
\]
where the right-hand side is $\beta$ times the cost of the fractional solution $x$.
It remains to relate the left side of this inequality with $ \mathbb{E}[\max_{p} Y_{p}]$.
%We observe that, in expectation, the cost of evicting each page is no more than $\beta$ times the cost of the fractional solution. However, since we are taking the maximum over all pages, we need to bound $\mathbb{E}[\max_{p} \sum_{j}Y_{p,j}]$.

\begin{lemma}
  Let $Y_{p,j}$ be Bernoulli random variables which are $1$ with probability $y_{p,j}$. Let $Y_p = \sum_{j} Y_{p,j}$ and assume there are $n$ such sums, then
  \[
    \mathbb{E}[\max_{p} Y_{p}] \le e \cdot \max_{p} E[Y_{p}] + \log(n).
  \]
\end{lemma}
\begin{proof}
  Let $Y = \max_{p} Y_{p}$. Using Jensen's inequality, we get the first inequality in the following chain of inequalities:
  \begin{align*}
    \exp(\mathbb{E}[Y]) &\le \mathbb{E}[\exp(Y)] = \mathbb{E}[\max_{p} \exp(Y_{p})] \\
    & \le \sum_{p} \mathbb{E}[\exp(Y_{p})]
    = \sum_{p} \prod_{j=1}^{r(p,T)} \mathbb{E}[\exp(Y_{p,j})] \\
    &= \sum_{p} \prod_{j=1}^{r(p,T)} (1 - y_{p,j} + e y_{p,j})
    \le \sum_{p} \prod_{j=1}^{r(p,T)} e^{e \cdot y_{p,j}}\\
    &= \sum_{p} e^{e \cdot \sum_{j=1}^{r(p,T)} y_{p,j}} \le n \cdot \max_{p} e^{e \cdot \mathbb{E}[Y_{p}]}.
  \end{align*}
  The first equality follows as $\exp$ is a monotone function, and the second equality follows by the independence of the $Y_{p,j}$.
  After taking logarithms, we obtain
  \[
    \mathbb{E}[Y] \le e \cdot \max_{p} \mathbb{E}[Y_{p}] + \log(n),
  \]
  which yields the desired result.
\end{proof}

Therefore, by the above lemma, the expected cost of the first type of costs is bounded by
\begin{equation}\label{type1costs}
 \mathbb{E}[\max_{p} Y_{p}] \le  O(1) \cdot \beta \max_p \sum_{j=1}^{r(p,T)} x_{p,j}.
\end{equation}

\begin{lemma}[\cite{bansal2021efficient}]\label{evictions}
Let $x$ be a fractional solution for a general paging problem. The expected cost of resets is at most $16 k e^{-\beta/4} \cdot\sum_{p \in P} \sum_{j=1}^{r(p,T)} x_{p,j}$.
\end{lemma}
%Note that  $16 k e^{-\beta/4} \cdot\sum_{p \in P} \sum_{j=1}^{r(p,T)} x_{p,j} \le 16 k e^{-\beta/4} \cdot n \max_p \sum_{j=1}^{r(p,T)} x_{p,j}.$
%Setting $\beta = 4( \log n + \log k)$ it follows that the cost for all evictions in Line 6is at most $16 k$ times the 

By choosing $\beta = 4\log(nk)$ in Lemma~\ref{evictions}, the expected total cost of resets for the solution $y$ becomes
\begin{equation}\label{type2costs}
16k e^{-\log(nk)} \sum_{p \in P} \sum_{j=1}^{r(p,T)} y_{p,j} \le \frac{16}{n} \sum_{p \in P} \sum_{j=1}^{r(p,T)} y_{p,j} \le \frac{16\beta}{n} \sum_{p\in P} \sum_{j=1}^{r(p,T)} x_{p,j} \le 16 \beta \max_{p \in P} \sum_{j=1}^{r(p,T)} x_{p,j}
\end{equation}
where the last inequality follows due to the fact that the average cost per page $\frac1n \sum_{p\in P} \sum_{j=1}^{r(p,T)} x_{p,j}$ is a lower bound on the maximum cost of a single page in the solution $x$.

Crucially, Lemma~\ref{evictions} depends on the following helper lemma: %, the proof of which is deferred to the Appendix:

\begin{restatable}{lemma}{roundinghelper}
\label{roundinghelper}
  Given a fractional solution $x$ to the paging problem, we can find a fractional solution $x^{*}$ in which every variable is a multiple of $\delta = \frac{1}{4k}$, and the cost of which is no more than $3$ times the cost of $x$.
\end{restatable}

% Recall that the first type of costs is bounded by $\beta \max_{p} \sum_{j=1}^{r(p,T)} x_{p,j}$, so with our choice of $\beta$, we obtain the following:

Taking the bounds on the two types of costs, namely Equations~\eqref{type1costs}~and~\eqref{type2costs}, we have shown the following:

\randomizedfinal*

% \begin{theorem}
%   There exists an $O(\log^{2}n \log k)$-competitive randomized integral algorithm for min-max paging.
% \end{theorem}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app_randlb.tex <==
\subsection{Randomized Lower Bound: $k \ge 2$}
(Work in progress - Max)

\begin{thm}\label{thm_rlb}
  The randomized competitive ratio of min-max paging is
  $\Omega(\log(k+1) \log_{k+1} n) = \Omega(\log n)$, where $n$ is the number of
  pages and $k$ is the size of the cache.
\end{thm}

By Yao's principle, it suffices to exhibit a probability distribution on input
instances which forces every deterministic online algorithm to perform a factor
$\Omega(\log n)$ worse in expectation as compared to the optimum cost. Let
$n=(k+1)^m$ for some large integer $m$. Our randomized adversarial strategy
takes a parameter $N \gg n$ and is defined as follows.
\begin{algorithm}
  \caption{An adversarial input distribution for min-max paging}\label{adversary}
  \begin{algorithmic}
    \State Let $L_m=\{p^m_0,\ldots,p^m_{n-1}\}$ be a set of $n=(k+1)^m$ pages.
    \For{$\ell$ $=$ $m$ to $1$} \State $L_{\ell-1}\gets\emptyset$.  \For{$i$ $=$
      $0$ to $(k+1)^{\ell-1}-1$} \State Give $N$ requests, chosen uniformly and
    independently at random from the set of pages
    $p^{\ell}_{(k+1)i},p^{\ell}_{(k+1)i+1}, \dots, p^{\ell}_{(k+1)i+k}$.  \State
    $p^{\ell-1}_i$ $\gets$ a uniformly random page from
    $p^{\ell}_{(k+1)i},p^{\ell}_{(k+1)i+1}, \dots, p^{\ell}_{(k+1)i+k}$.  \State
    Add $p^{\ell-1}_i$ to $L_{\ell-1}$.  \EndFor \EndFor
  \end{algorithmic}
\end{algorithm}

We call each iteration of the outer for-loop a \textit{layer} and each of the
inner for-loop a \textit{phase}. We number layers $m,m-1,\ldots,1$.

Let $X_{i}^\ell$ be the number of faults incurred by page $p_i^\ell$ at the
beginning of layer $\ell$.

\begin{lem}
  For every layer $\ell$ and every $i \in \{0, (k+1)^\ell - 1\}$ we have
  $\mathbb{E}[X_i^\ell] \ge (m-l) \cdot N/(k+1)^2$.
\end{lem}
\begin{proof}
  We will prove this by reverse induction on the number of layers. We observe
  that $X_i^m = 0$ for all $i \in \{0, n-1\}$. Assume now that we have shown for
  each $i \in \{0, 1, \dots, (k+1)^\ell-1\}$ that
  $\mathbb{E}[X_i^\ell] \ge (m-\ell) \frac{N}{(k+1)^2}$. We will prove that for
  every $j \in \{0, 1, \dots, (k+1)^{\ell-1} - 1\}$ we have
  $\mathbb{E}[X_i^\ell] \ge (m-\ell+1) \frac{N}{(k+1)^2}$.

  During the $j$th phase of layer $\ell$ we give $N$ requests chosen uniformly
  at random from a set of $k+1$ pages. This means that any algorithm for min-max
  paging with a cache of size $k$ faults exactly when the page that is not in
  its cache at a given point in time is chosen for the next request. This
  happens with probability $\frac{1}{k+1}$ and so, by linearity of expectation,
  the algorithm will fault $\frac{N}{k}$ times in expectation. Let $Y_i^\ell$
  denote the number of page faults for a single page $p_i^\ell$ during the $j$th
  phase. At the end of the phase, we choose one of the pages uniformly at
  random, so the expected number of faults on this page, which will be
  $X_{j}^{\ell-1}$, becomes
  \begin{align*}
    \mathbb{E}[X_j^{\ell-1}] &\ge \sum_{i=0}^{k} \frac{1}{k+1} \mathbb{E}[X_{(k+1)j+i}^\ell] + \sum_{i=0}^{k} \frac{1}{k+1} \mathbb{E}[Y_i^\ell] \\
                             & = (m-\ell) \frac{N}{(k+1)^2} + \frac{N}{(k+1)^2} = (m - \ell + 1) \frac{N}{(k+1)^2}.
  \end{align*}
  The first term in the inequality is due to the induction hypothesis and the
  second term comes from the faults incurred during the current phase.
\end{proof}

By holding on to the page that will be moved on to the next layer and employing
the GreedyLFD strategy on the remaining $k$ pages with $k-1$ cache slots, we
find that OPT has cost $m + 4N / (k(k+1) H_{k+1})$.

\begin{lem}
  Assume $\sigma$ is a request sequence of length $T$ where each request is
  chosen uniformly at random from the set $p_1, p_2, \dots, p_{k+1}$. Then the
  cost of OPT for min-max paging on this request sequence is at most
  $4T / (k(k+1) H_{k+1})$.
\end{lem}
\begin{proof}
  We want to bound the expected number of requests needed to increase the cost
  of OPT, using the algorithm GreedyLFD. As in the deterministic case, we
  consider the variables $T_i$, which are now random variables, and denote the
  round during which $\max_{p \in P} \cost(GreedyLFD, \sigma, p, t)$ first
  reaches $i$.

  We note that $T_1 = 1$, as the algorithm GreedyLFD always starts with an empty
  cache. For $T_2$, we note that in expectation, it will be greater than
  $2 (k+1) H_{k+1}$, by the coupon collector's problem, as we need to request
  each page once to incur the first fault on each page, and subsequently, we
  need to request all pages again, before faulting for the second time on any
  page. This is because GreedyLFD, upon having seen all $k+1$ pages, will eject
  the page that comes last out of all of them, which next occurs after
  $(k+1) H_{k+1}$ time steps, in expectation.

  For general $i$, we will now show that
  $\mathbb{E}[T_{i+1}] \ge \frac{k(k+1}{4} (2H_{k+1} - 1) + E[T_{i}]$. Let us
  fix $i$ and assume we are currently at time $T_i$. That means there is one
  page of cost $i$ and all other pages are of cost less than $i$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm_rlb}]
  Take ratios between them
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

